Outward Influence and Cascade Size Estimation in Billion-scale Networks

Estimating cascade size and nodes' influence is a fundamental task in social, technological, and biological networks. Yet this task is extremely challenging due to the sheer size and the structural heterogeneity of networks. We investigate a new influence measure, termed outward influence (OI), defined as the (expected) number of nodes that a subset of nodes $S$ will activate, excluding the nodes in S. Thus, OI equals, the de facto standard measure, influence spread of S minus |S|. OI is not only more informative for nodes with small influence, but also, critical in designing new effective sampling and statistical estimation methods. Based on OI, we propose SIEA/SOIEA, novel methods to estimate influence spread/outward influence at scale and with rigorous theoretical guarantees. The proposed methods are built on two novel components 1) IICP an important sampling method for outward influence, and 2) RSA, a robust mean estimation method that minimize the number of samples through analyzing variance and range of random variables. Compared to the state-of-the art for influence estimation, SIEA is $\Omega(\log^4 n)$ times faster in theory and up to several orders of magnitude faster in practice. For the first time, influence of nodes in the networks of billions of edges can be estimated with high accuracy within a few minutes. Our comprehensive experiments on real-world networks also give evidence against the popular practice of using a fixed number, e.g. 10K or 20K, of samples to compute the "ground truth" for influence spread.

==> body/extension.tex <==
%\section{Dynamic Algorithm}
%\label{sec:extension}
%%One of the difficulties appears when developing \PIMA{} is how we can select the values of $\epsilon_1, \epsilon_2, \epsilon_3$ as well as $\delta_1$ and $\delta_2$. We want to have a setting that minimizes the number of RR sets generated in both the main and \textsf{Estimate-Influence} procedures. In Section \ref{sec:approx}, we formed the intuition of how their values would impact the running time and by experimenting with various assignments, we find a set of three values that robustly give good performance. However, that is not a guarantee. To address that problem, 
%
%In this section, we propose the dynamic algorithm, named \DPIMA{}, that automatically selects $\epsilon_1, \epsilon_2, \epsilon_3, \delta_1, \delta_2$ during its execution. While maintaining the $(1-1/e-\epsilon)$-approximate solution as in \PIMA{}, \DPIMA{} requires, to within a constant factor, the type-2 minimum threshold. This is the strongest result over all \IM{} methods following the \RIS{} framework.
%\subsection{D-SSA Algorithm}
%
%In Section \ref{sec:alg}, \PIMA{} can be seen as generating two independent collections of RR sets: one is in the main algorithm to find the maximum seed set and the another is for estimating the influence of the seed set found in the main procedure. Recall from Section \ref{sec:approx} that we want to start checking the influence of $\hat S_k$ at the moment of having generated just enough RR sets so that the RR sets for checking are not wasted. However, detecting that moment is challenging since it depends not only on the networks but also the particular execution of generating RR sets.
% \begin{algorithm}[!ht]
% 	\caption{\DPIMA{} Algorithm}
% 	\label{alg:dpima}
% 	\KwIn{Graph $G$, $0 \leq \epsilon, \delta \leq 1$, and $k$}
% 	\KwOut{An $(1 - 1/e - \epsilon)$-optimal solution, $\hat S_k$}
% 	$\Lambda \leftarrow (1 + \epsilon)^2\Upsilon(\epsilon,\delta/2)$\\
% 	$\R \leftarrow$ Generate $\Lambda$ random RR sets by \RIS{}\\
% 	$<$$\hat S_k,\hat \I(\hat S_k)$$>\leftarrow$ \textsf{Max-Coverage}($\R,k$)\\
% 	\Repeat{$|\R|\geq (2+\frac{2\epsilon}{3})n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{k\epsilon^2}$ (from Eq.~\ref{eq:theta_2})}{
% 		$\R' \leftarrow$ Generate $|\R|$ random RR sets by \RIS{}\\
% 		$\I_{c}(\hat S_k) \leftarrow \Cov_{\R'}(\hat S_{k})\cdot n/|\R'|$\\
% 		$\epsilon_1 \leftarrow \hat \I(\hat S_k)/\I_{c}(\hat S_k) - 1$\\
% 		\If{$(\epsilon_1 \leq \epsilon)$}{
% 			$\epsilon_2 \leftarrow \frac{\epsilon-\epsilon_1}{2(1+\epsilon_1)}$, $\epsilon_3 \leftarrow \frac{\epsilon-\epsilon_1}{2(1-1/e)}$\\
% 			$\delta_1 \leftarrow e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{(2+2/3\epsilon_3)(1+\epsilon_1)(1+\epsilon_2)}}$\\
% 			$\delta_2 \leftarrow e^{-\frac{(\Cov_{\R'}(\hat S_k)-1)\cdot \epsilon_2^2}{(2+2/3\epsilon_2)(1+\epsilon_2)} + \ln [2 \log_2 n]}$\\
% 			\If{$\delta_1+\delta_2\leq \delta$}{
% 				\textbf{return} $\hat S_k$
% 			}
% 		}
% 		$\R \leftarrow \R \cup \R'$ \\
% 		$<$$\hat S_k,\hat \I(\hat S_k)$$>\leftarrow$ \textsf{Max-Coverage}($\R,k$)
% 	}
% 	\textbf{return} $\hat S_k$
% \end{algorithm}
%
%The dynamic algorithm \DPIMA{}, described in Alg.~\ref{alg:dpima}, addresses thoroughly these issue by dynamically computing the values of $\epsilon_1, \epsilon_2, \epsilon_3, \delta_1, \delta_2$ along its execution and stops whenever the success probability meets the requirement (Line 12). \DPIMA{} also reuses the checking RR sets for finding seed set without affecting the independence of RR sets in subsequent iterations (Line 16). More specifically, \DPIMA{} uses the newly generated RR sets to estimates the influence of the seed set found in the previous iteration and obtain the current value of $\epsilon_1$ (Line 7). From the value of $\epsilon_1$, $\epsilon_2$ and $\epsilon_3$ can be computed accordingly (Line 8). The formula for computing $\epsilon_2$ and $\epsilon_3$ are based on the condition that
%\begin{align}
%	\epsilon_1 + \epsilon_2 + \epsilon_1\epsilon_2 + \epsilon_3(1-1/e) \leq \epsilon
%\end{align}
%\noindent and considering $\epsilon_2 + \epsilon_1\epsilon_2$ and $\epsilon_3(1-1/e)$ having similar roles. After that it relies on the two stopping conditions mentioned in \PIMA{} to calculate $\delta_1$ and $\delta_2$. \DPIMA{} stops when sum of $\delta_1$ and $\delta_2$ is less than or equal to $\theta$ which signifies that the success probability meets the requirement.
%
%%degree of $\hat S_k$ at the current iteration, $\epsilon_3$ is also computable and finally, $\epsilon_2$ is calculated from $\epsilon, \epsilon_1$ and $\epsilon_3$. Based on $\epsilon_2$, we can obtain an estimate of the number of RR sets needed in the calculating influence procedure and compare that with the generated RR sets: if it is greater, we do not check and continue doubling strategy, otherwise, we check the influence and recompute $\epsilon_1, \epsilon_2, \epsilon_3$. The algorithm finishes when Eq. \ref{eq:epsilon} holds.
%
%%Notice the checking $( d_{\epsilon_2} \frac{|\mathcal E'|}{deg_{\mathcal E'}(S_{old})} \leq 2|\mathcal E|)$ (Line 17): the left side is the estimated number of samples to compute influence based on the estimation of $S_{old}$. Since we allow the checking to have a constant times the number of RR sets in the main algorithm and estimating $\I(S_{old})$ only uses half of that number. Thus, the approximation factor of $\hat \I(S_{old})$ may be $\sqrt{2}$ times worse and to account for that, we multiply $2$ in the right hand side.
%
%\subsection{D-SSA Analysis}
%We will sequentially show that \DPIMA{} achieves $(1-1/e-\epsilon)$-approximation factor in Subsec.~\ref{subsub:dima_approx} and requires only, to within a constant factor, the strongest type-2 minimum threshold of the RR sets in Subsec.~\ref{subsub:dima_rr}.
%\subsubsection{Approximation Guarantee}
%\label{subsub:dima_approx}
%We show that \DPIMA{} preserve the $(1-1/e-\epsilon)$-approximation factor of \PIMA{} by the following theorem.
%\begin{theorem}
%	Given a graph $G$, $0\leq \epsilon \leq 1-2/e$ and $0\leq \delta \leq 1$ as the inputs, \DPIMA{} returns a $(1-1/e-\epsilon)$-approximate solution.
%\end{theorem}
%\begin{proof}
%	we prove that the two stopping conditions in \PIMA{} are still hold in \DPIMA{} and thus \DPIMA{} has the same approximation factor as \PIMA{} does.
%	
%	Directly from the Alg.~\ref{alg:dpima}, when \DPIMA{} terminates, the following conditions are satisfied,
%	\begin{align}
%		\label{eq:eq7}
%		\Cov_{\R}(\hat S_k) = (2+\frac{2}{3}\epsilon_3)(1+\epsilon_1)(1+\epsilon_2)\ln \frac{1}{\delta_1}\frac{1}{\epsilon_3^2}
%	\end{align}
%	\vspace{-0.2in}
%	
%	\noindent and
%	\vspace{-0.05in}
%	\begin{align}
%		\label{eq:eq8}
%		\Cov_{\R'}(\hat S_k) = 1+(2+\frac{2}{3}\epsilon_2)(1+\epsilon_2)\ln \frac{2 \log_2 n}{\delta_2}\frac{1}{\epsilon_2^2}
%	\end{align}
%	\noindent with $\epsilon_1 + \epsilon_2 + \epsilon_1\epsilon_2 + (1-1/e)\epsilon_3 = \epsilon$ and $\delta_1 + \delta_2 = \delta$.
%	
%	Eq.~\ref{eq:eq7} is the first stopping conditions in \PIMA{}. Eq.~\ref{eq:eq8} is the checking condition in the \textsf{Estimate-Inf} procedure in \PIMA{} and, together with the setting of $\epsilon_1$, we obtain the second stopping condition in \PIMA{}.
%	\begin{align}
%		\hat \I(\hat S_k) \geq (1+\epsilon_1)(1+\epsilon_2) \I(\hat S_k)
%	\end{align}
%	Thus, the $(1-1/e-\epsilon)$-approximation factor is followed from \PIMA{} which completes the proof.
%\end{proof}
%
%\subsubsection{Achieving the Type-2 Minimum Threshold}
%\label{subsub:dima_rr}
%Here, we will prove a much stronger result than that of \PIMA{} that \DPIMA{} requires only, to within a constant factor, the type-2 minimum of RR sets $N^2_{min}(\epsilon, \delta)$. Since $\epsilon^*_a \leq \epsilon$ and $\delta^*_b \leq \delta$, let denote the constant
%\begin{align}
%	M = \frac{\ln\frac{2}{\delta^*_b}}{\ln \frac{1}{\delta^*_b}}\frac{8 \cdot (1+\epsilon) \cdot(1+\epsilon^*_a)^2}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^3} \leq \frac{\ln\frac{2}{\delta}}{\ln \frac{1}{\delta}}\frac{8 \cdot(1+\epsilon)^3}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^3}
%\end{align}
%\noindent Alternatively speaking, for a given graph $G$, we will show that \DPIMA{} terminates when the number of RR sets in $\R$ is larger than or equal to $M\textsf{c}_1N^2_{min}(\epsilon, \delta)$, where $\textsf{c}_1$ is a constant defined in Lem. \ref{lem:zo}, with at least $(1-\delta)$-probability. Due to the doubling scheme, \DPIMA{} will generate no more than twice that number. More specifically, we will prove that the stopping condition (Line 11) is satisfied.  Recall $N^2_{min}(\epsilon, \delta)$ RR sets implies,
%	\begin{align}
%		\label{eq:given1}
%		\Pr[\hat \I(\hat S_k) \leq (1 + \epsilon^*_a) \I(\hat S_k)] \geq 1-\delta^*_a
%	\end{align}
%	\vspace{-0.2in}
%	
%	\noindent and
%	\begin{align}
%	\label{eq:given2}
%		\Pr[\hat \I(S^*_k) \geq (1 - \epsilon^*_b)OPT_k] \geq 1 - \delta^*_b
%	\end{align}
%	\vspace{-0.2in}
%	
%	\noindent where
%	\begin{align}
%		N^1_{min}(\epsilon^*_a,\epsilon^*_b,\delta^*_a,\delta^*_b) = \min_{\epsilon_a,\epsilon_b,\delta_a,\delta_b}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b) \nonumber
%	\end{align}
%	\noindent Apply Theo.~\ref{theo:type1}, we have
%	\begin{align}
%		\label{eq:given3}
%		\Pr[\I(\hat S_k) \geq (1-1/e-\epsilon)OPT_k] \geq 1-\delta
%	\end{align}
%%	First, we prove a new approximation of $\I(S^*_k)$, in case of having $\frac{4 \cdot(1+\epsilon^*_a)^2(1-1/e)(1-\epsilon^*_b/2)\textsf{c}_1}{(1/2-1/e-\epsilon/2)^2}\Theta^*(\epsilon,\delta)$ RR sets.
%%	
%%	\begin{Lemma}
%%		\label{lem:theta_opt}
%%		When the number of RR sets in \DPIMA{} $|\R| \geq \frac{4 \cdot(1+\epsilon^*_a)^2(1-1/e)(1-\epsilon^*_b/2)\textsf{c}_1}{(1/2-1/e-\epsilon/2)^2}\Theta^*(\epsilon,\delta)$, then,
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\Pr[\hat \I(S^*_k) \geq (1 - \epsilon^*_b/2)OPT_k] \geq 1 - \delta^*_b/3
%%		\end{align} 
%%		\vspace{-0.25in}
%%	\end{Lemma}
%%	
%%	\begin{proof}
%%		Let $X^* = \min\{1, |I(S^*_k)/n$. Apply Lem. \ref{lem:zo} on the approximation of $\mu_{X^*}$ to achieve Eq.~ \ref{eq:given2},
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\frac{\Upsilon(\epsilon^*_b,\delta^*_b/3)}{\mu_{X^*}} \leq \textsf{c}_1 \Theta^*(\epsilon,\delta)
%%		\end{align}
%%		\vspace{-0.2in}
%%	\end{proof}
%	First, we show that the value of $\epsilon_1$ is upper bounded by the following lemma.
%	\begin{Lemma}
%		\label{lem:epsilon_dima}
%		Given $0\leq \epsilon \leq 1-2/e$ and $0\leq \delta \leq 1$, if $|\R| \geq M\textsf{c}_1N^2_{min}(\epsilon, \delta)$, then,
%		\begin{align}
%			\Pr[\epsilon_1 \leq \frac{\epsilon^*_a + \epsilon^*_b/2}{1 - \epsilon^*_b/2}] \geq 1 - \delta
%		\end{align}
%		\noindent where $\textsf{c}_1$ is a constant defined in Lem.~\ref{lem:zo}.
%	\end{Lemma}
%%	\begin{proof}
%%		To prove the lemma, we begin by showing that $\I(S^*_k)$ has an better approximation when $|\R| \geq M\textsf{c}_1N^2_{min}(\epsilon, \delta)$. Let $X^* = \min\{1, |R_j \cap S^*_k|\}$ ($R_j$ is a random RR set) be a random variable with $\mu_{X^*} = OPT_k/n$. Apply Lem. \ref{lem:zo} on the approximation of $\mu_{X^*}$ to achieve Eq.~ \ref{eq:given2}, we have
%%		\vspace{-0.05in}
%%		\begin{align}
%%			\frac{\Upsilon(\epsilon^*_b,\delta^*_b)}{\mu_{X^*}} \leq \textsf{c}_1 N^2_{min}(\epsilon, \delta)
%%		\end{align}
%%		\vspace{-0.2in}
%%%		
%%%		\noindent or, equivalently,
%%%		\vspace{-0.1in}
%%%		\begin{align}
%%%			2c\ln\frac{1}{\delta^*_b}\frac{n}{\epsilon^{*2}_b OPT_k} \leq \textsf{c}_1 \Theta^*(\epsilon,\delta)
%%%		\end{align}
%%%		\vspace{-0.15in}
%%		
%%		\noindent Multiply both sides by $M$, we have
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\frac{M\Upsilon(\epsilon^*_b,\delta^*_b)}{\mu_{X^*}} \leq M\textsf{c}_1N^2_{min}(\epsilon, \delta)
%%		\end{align}
%%		\vspace{-0.15in}
%%		
%%		\noindent In other words,
%%		\vspace{-0.15in}
%%		\begin{align}
%%			\label{eq:new_set}
%%			|\R| \geq \frac{M\Upsilon(\epsilon^*_b,\delta^*_b)}{\mu_{X^*}}
%%		\end{align}
%%		\vspace{-0.25in}
%%		
%%		\noindent Then, since 
%%		\vspace{-0.1in}
%%		\begin{align}
%%			M\Upsilon(\epsilon^*_b,\delta^*_b)=\frac{\ln\frac{2}{\delta^*_b}}{\ln \frac{1}{\delta^*_b}}\frac{4(1+\epsilon^*_a)^2}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^3} \Upsilon(\epsilon^*_b,\delta^*_b) \geq \Upsilon(\frac{\epsilon^*_b}{2},\frac{\delta^*_b}{2}), \nonumber
%%		\end{align}
%%		\vspace{-0.25in}
%%		
%%		\noindent thus,
%%		\vspace{-0.15in}
%%		\begin{align}
%%			\label{eq:new_set_2}
%%			|\R| \geq \frac{\Upsilon(\frac{\epsilon^*_b}{2},\frac{\delta^*_b}{2})}{\mu_{X^*}}
%%		\end{align}
%%		\vspace{-0.15in}
%%		
%%		Apply Lem.~\ref{lem:zo} with the number of RR sets specified in Eq.~\ref{eq:new_set_2}, we have
%%		\vspace{-0.05in}
%%		\begin{align}
%%			\label{eq:eq9}
%%			\Pr[\hat \I(S^*_k) \geq (1 - \epsilon^*_b/2)OPT_k] \geq 1 - \delta^*_b/2
%%		\end{align} 
%%		\vspace{-0.2in}
%%		
%%		\noindent Combine Eq.~\ref{eq:given1} and Eq.~\ref{eq:eq9} and apply Theo.~\ref{theo:type1},
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\label{eq:new_approx}
%%			\Pr[\I(\hat S_k) \geq (1-\frac{1}{e}-\epsilon)OPT_k] \geq 1-\delta^*_a - \frac{\delta^*_b}{2}
%%		\end{align}
%%		\vspace{-0.2in}
%%		
%%		In Eq. \ref{eq:new_set}, $|\R|$ depends on $\mu_{X^*} = OPT_k/n$ and in Eq. \ref{eq:new_approx}, we obtained the relation between $\I(\hat S_k)$ and $OPT_k$ and, thus, we can represent $|\R|$ in terms of $\I(\hat S_k)$,
%%		\vspace{-0.15in}
%%		\begin{align}
%%			\Pr[|\R| \geq \frac{M\Upsilon(\epsilon^*_b,\delta^*_b)(1-1/e-\epsilon)}{\I(\hat S_k)/n}] \geq 1-\delta^*_a - \frac{\delta^*_b}{2} \nonumber
%%		\end{align}
%%		\vspace{-0.15in}
%%		
%%		\noindent and since $M\Upsilon(\epsilon^*_b,\delta^*_b)(1-1/e-\epsilon) \geq \Upsilon(\frac{\epsilon^*_b}{2},\frac{\delta^*_b}{2})$,
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\label{eq:num_rr}
%%			\Pr[|\R| \geq \frac{\Upsilon(\frac{\epsilon^*_b}{2},\frac{\delta^*_b}{2})}{\I(\hat S_k)/n}] \geq 1-\delta^*_a - \frac{\delta^*_b}{2}
%%		\end{align}
%%		\vspace{-0.15in}
%%%		\begin{align}
%%%			\textsf{a}\cdot \Theta^*(\epsilon,\delta) \geq 2c\ln\frac{2}{\delta^*_b}\frac{n\cdot (1-\epsilon^*_b)}{\epsilon^{*2}_b \hat \I(S^*_k)}
%%%		\end{align}
%%%		\vspace{-0.15in}
%%		
%%		Notice that in each iteration \DPIMA{} generates $|\R|$ new random RR sets and put them in $\R'$ to compute $\I_c(\hat S_k)$. Thus, 
%%		\vspace{-0.15in}
%%		\begin{align}
%%			\label{eq:num_rr'}
%%			\Pr[|\R'| \geq \frac{\Upsilon(\frac{\epsilon^*_b}{2},\frac{\delta^*_b}{2})}{\I(\hat S_k)/n}] \geq 1-\delta^*_a - \frac{\delta^*_b}{2}
%%		\end{align}
%%		\vspace{-0.15in}
%%		
%%		\noindent In the cases that $|\R'| \geq \frac{\Upsilon(\frac{\epsilon^*_b}{2},\frac{\delta^*_b}{2})}{\I(\hat S_k)/n}$, apply Lem.~\ref{lem:zo},
%%		\vspace{-0.05in}
%%		\begin{align}
%%			\Pr[\I_c(\hat S_k) \geq (1 - \epsilon^*_b/2)\I(\hat S_k)] \geq 1 - \delta^*_b/2
%%		\end{align} 
%%		\vspace{-0.2in}
%%		
%%		\noindent Combine with the probability in Eq.~\ref{eq:num_rr'}, we have
%%		\vspace{-0.05in}
%%		\begin{align}
%%			\Pr[\I_c(\hat S_k) \geq (1 - \epsilon^*_b/2)\I(\hat S_k)] \geq 1 - \delta^*_a - \delta^*_b
%%		\end{align} 
%%		\vspace{-0.2in}
%%		
%%		\noindent or, equivalently,
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\label{eq:new_app}
%%			\Pr[\I(\hat S_k) \leq \frac{1}{1 - \epsilon^*_b/2}\I_c(\hat S_k)] \geq 1 - \delta^*_a - \delta^*_b
%%		\end{align} 
%%		\vspace{-0.2in}
%%		
%%		\noindent Thus, from Eq.~\ref{eq:given1} and Eq.~\ref{eq:new_app} with a note that Eq.~\ref{eq:given1} was used to derive Eq.~\ref{eq:new_app} and, thus, the probability that both happen is actually the probability in Eq.~\ref{eq:new_app}, we achieve
%%		\vspace{-0.05in}
%%		\begin{align}
%%			\label{eq:eq10}
%%			\Pr[\hat \I(\hat S_k) \leq \frac{1 + \epsilon^*_a}{1-\epsilon^*_b/2} \I_c(\hat S_k)] \geq 1 - \delta^*_a - \delta^*_b
%%		\end{align} 
%%		\vspace{-0.15in}		
%%		
%%		\noindent Then, since $\epsilon_1 = \frac{\hat \I(\hat S_k)}{\I_c(\hat S_k)} -1$ and from Eq.~\ref{eq:eq10},
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\Pr[\epsilon_1 \leq \frac{1 + \epsilon^*_a}{1 - \epsilon^*_b/2}-1] \geq 1 - \delta^*_a - \delta^*_b
%%		\end{align} 
%%		\vspace{-0.2in}
%%		
%%		\noindent and due to $\delta^*_a + \delta^*_b \leq \delta$,
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\Pr[\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}] \geq 1-\delta
%%		\end{align} 
%%		\vspace{-0.15in}
%%		
%%		\noindent which completes the proof.
%%		\end{proof}
%		
%		The proof is presented in the appendix. Based on the result of Lem.~\ref{lem:epsilon_dima}, we next prove that \DPIMA{} will terminate when $|\R| \geq M\textsf{c}_1N^2_{min}(\epsilon, \delta)$ with at least $(1-\delta)$-probability.
%		\begin{Lemma}
%			\label{lem:2}
%			If $|\R| \geq M\textsf{c}_1N^2_{min}(\epsilon, \delta)$ and $\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}$, then,
%			\begin{align}
%			\delta_1 + \delta_2 \leq \delta
%			\end{align}
%		\end{Lemma}
%%		\begin{proof}
%%			 Notice that since $\epsilon \leq 1-2/e$, we have $\frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2} \leq \epsilon$ and the condition in Line 9 is satisfied. Given $\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}$, we compute $\epsilon_2, \epsilon_3$ as,
%%			\vspace{-0.1in}
%%			\begin{align}
%%				\label{eq:e2}
%%				\epsilon_2 = \frac{\epsilon-\epsilon_1}{2(1+\epsilon_1)} \geq \frac{1/2-1/e-\epsilon/2}{1+\epsilon^*_a}\frac{\epsilon^*_b}{2}
%%			\end{align}
%%			\vspace{-0.25in}
%%			
%%			\noindent and
%%			\vspace{-0.1in}
%%			\begin{align}
%%				\label{eq:e3}
%%				\epsilon_3 = \frac{\epsilon-\epsilon_1}{2(1-1/e)} \geq (1/2-1/e-\epsilon/2)\frac{\epsilon^*_b}{2}
%%			\end{align}
%%			\vspace{-0.15in}
%%			
%%			Since $\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}$ also implies that all the inequality used in the proof of Lem. \ref{lem:epsilon_dima} hold, then
%%			\vspace{-0.05in}
%%			\begin{align}
%%				\hat \I(S^*_k) \geq (1 - \epsilon^*_b/2)OPT_k
%%			\end{align}
%%			\vspace{-0.2in}
%%			
%%			\noindent Combine with $\hat \I(\hat S_k) \geq (1-1/e)\hat \I(S^*_k)$, we have
%%			\vspace{-0.05in}
%%			\begin{align}
%%				\hat \I(\hat S_k) \geq (1-1/e)(1 - \epsilon^*_b/2)OPT_k
%%			\end{align}
%%			\vspace{-0.2in}
%%			
%%			\noindent Replace $OPT_k$ in $\mu_{X^*} = OPT_k/n$ by that in the above inequality, we get $\mu_{X^*} \leq \frac{\hat \I(\hat S_k)}{n(1-1/e)(1 - \epsilon^*_b/2)} \leq \frac{\hat \I(\hat S_k)}{n(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})}$ and then the number of RR sets in Eq.~\ref{eq:new_set} is rewritten as,
%%			\vspace{-0.15in}
%%			\begin{align}
%%				|\R| \geq \frac{\ln\frac{2}{\delta^*_b}}{\ln \frac{1}{\delta^*_b}}\frac{4(1+\epsilon^*_a)^2}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^2}\frac{\Upsilon(\epsilon^*_b,\delta^*_b)}{\hat \I(\hat S_k)/n}
%%			\end{align}
%%			\vspace{-0.2in}
%%			
%%			\noindent or, equivalently,
%%			\vspace{-0.1in}
%%			\begin{align}
%%				|\R|\frac{\hat \I(\hat S_k)}{n} \geq 2c\ln \frac{2}{\delta^*_b}\frac{4(1+\epsilon^*_a)^2}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^2\epsilon^{*2}_b} \geq 2c\ln \frac{2}{\delta^*_b}\frac{1}{\epsilon^{*2}_b} \nonumber
%%			\end{align}
%%			\vspace{-0.15in}
%%			
%%			\noindent The left hand side is the coverage of $\hat S_k$ in $\R$, $\Cov_{\R}(\hat S_k)$. Combining that and the calculated $\epsilon_1,\epsilon_2,\epsilon_3$ to find $\delta_1$,
%%			\vspace{-0.1in}
%%			\begin{align}
%%				\label{eq:d1}
%%				\delta_1 = e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{2c(1+\epsilon_1)(1+\epsilon_2)}} \leq e^{-\frac{2c\ln \frac{2}{\delta^*_b}\frac{1}{\epsilon^2_3}\cdot \epsilon_3^2}{2c(1+\epsilon_1)(1+\epsilon_2)}} \leq \delta^*_b/2
%%			\end{align}
%%			\vspace{-0.2in}
%%			
%%			To compute the value of $\delta_2$, we base on the fact that $|\R'| = |\R|$ and Eq.~\ref{eq:num_rr'},
%%			\vspace{-0.1in}
%%			\begin{align}
%%				\label{eq:d2}
%%				\delta_2 = e^{-\frac{\Cov_{\R'}(\hat S_k)\cdot \epsilon_2^2}{2c(1+\epsilon_2)}} \leq e^{-\frac{2c\ln \frac{2}{\delta^*_b}\frac{1}{\epsilon^2_2}\cdot \epsilon_2^2}{2c(1+\epsilon_2)}} \leq \delta^*_b/2
%%			\end{align}
%%			\vspace{-0.2in}
%%			
%%			From Eq.~\ref{eq:d1} and Eq.~\ref{eq:d2}, we conclude
%%			\vspace{-0.1in}
%%			\begin{align}
%%				\delta_1 + \delta_2 \leq \delta^*_b/2 + \delta^*_b/2 = \delta^*_b \leq \delta
%%			\end{align}
%%			\vspace{-0.2in}
%%			
%%			\noindent which proves Lem. \ref{lem:2}.
%%%			\vspace{-0.05in}
%%%			\begin{align}
%%%				\label{eq:2}
%%%				\hat \I(\hat S_k) \leq (1 + \epsilon^*_a) \I(\hat S_k)
%%%			\end{align}
%%%			\vspace{-0.15in}
%%%			
%%%			\noindent Replace $\I(\hat S_k)$ in Eq. \ref{eq:1} by that from Eq. \ref{eq:2},
%%%			\vspace{-0.1in}
%%%			\begin{align}
%%%				\label{eq:3}
%%%				|\R| \geq 	\frac{\ln\frac{4}{\delta^*_b}}{\ln \frac{1}{\delta^*_b}}\frac{4(1+\epsilon^*_a)^2}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^2}\frac{\Upsilon(\epsilon^*_b,\delta^*_b)(1-1/e-\epsilon)}{\I(\hat S_k)/n}
%%%			\end{align}
%%%			\vspace{-0.2in}
%%%			
%%%			
%%%			\noindent Consequently, we can compute $\delta_1$ from $\epsilon_2, \epsilon_3$,
%%%			\vspace{-0.1in}
%%%			\begin{align}
%%%				\delta_1 = e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{2c(1+\epsilon_1)(1+\epsilon_2)}}
%%%			\end{align}
%%%			\vspace{-0.2in}
%%			
%%		\end{proof}
%		
%%		\vspace{-0.05in}
%%		\begin{align}
%%		\textsf{a}\cdot \Theta^*(\epsilon,\delta) \geq 2c\ln\frac{2}{\delta^*_b}\frac{n\cdot (1-\epsilon^*_b) (1-1/e)}{\epsilon^{*2}_b \hat \I(\hat S_k)}
%%		\end{align}
%%		\vspace{-0.2in}
%%		
%%		\noindent Thus,
%%		\vspace{-0.05in}
%%		\begin{align}
%%		%	\label{eq:com1}
%%		\frac{\hat \I(\hat S_k)\textsf{a}\cdot\Theta^*(\epsilon,\delta)}{n} \geq (1-\epsilon^*_b) (1-1/e)2c\ln\frac{2}{\delta^*_b}\frac{1}{\epsilon^{*2}_b}
%%		\end{align}
%%		\vspace{-0.15in}
%%		
%%		\noindent The term $\frac{\hat \I(\hat S_k)\textsf{a}\cdot\Theta^*(\epsilon,\delta)}{n}$ in the above inequality is actually the coverage of $\hat S_k$ ($\Cov_{\R}(\hat S_k)$) when $|\R| = \textsf{a}\cdot\Theta^*(\epsilon,\delta)$.
%%		
%	
%%	\noindent is constant times the optimal number of RR sets to achieve Eq. \ref{eq:given2}.  Multiply both side of the inequality with $\frac{4 \textsf{a}\cdot \Theta^*(\epsilon,\delta)(1+\epsilon)^2}{(1-\epsilon) (1-1/e)^3}$, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\label{eq:com1}
%%	\frac{\hat \I(\hat S_k)}{n} \frac{4 \textsf{a}\cdot\Theta^*(\epsilon,\delta)(1+\epsilon)^2}{(1-\epsilon) (1-1/e)^3} \geq \frac{4(1+\epsilon)^2}{(1-1/e)^2} 2c\ln\frac{2}{\delta^*_b}\frac{1}{\epsilon^{*2}_b}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	Furthermore, since \DPIMA{} always maintain $\hat \I(\hat S_k) \leq (1+\epsilon_1)(1+\epsilon_2)\I(\hat S_k)$ and when the number of RR sets exceeds $\Theta^*(\epsilon,\delta)$, we also have $\hat \I(\hat S_k) \leq (1+\epsilon^*_a)\I(\hat S_k)$,
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\epsilon_1 \leq \epsilon^*_a
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent which consequently leads to
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\epsilon_2 =\frac{\epsilon-\epsilon_1}{2(1+\epsilon_1)} \geq \frac{\epsilon-\epsilon^*_a}{2(1+\epsilon^*_a)}=\frac{1-1/e}{2(1+\epsilon^*_a)}\epsilon_b
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent and
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\epsilon_3 =\frac{\epsilon-\epsilon_1}{2(1-1/e)} \geq \frac{\epsilon-\epsilon^*_a}{2(1-1/e)}=\frac{\epsilon_b}{2}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	Now, apply Eq. \ref{eq:com1}, we can compute $\delta_1$ and $\delta_2$ with respect to $\epsilon_1, \epsilon_2, \epsilon_3$ obtained above when the number of RR sets is $|\R| = \frac{4 \textsf{a}\cdot(1+\epsilon)^2}{(1-\epsilon) (1-1/e)^3}\Theta^*(\epsilon,\delta)$,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\label{eq:delta1}
%%		\delta_1 = e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{2c(1+\epsilon_1)(1+\epsilon_2)}} \leq e^{-\frac{\frac{4(1+\epsilon)^2}{(1-1/e)^2}2c\ln\frac{2}{\delta^*_b}\frac{1}{\epsilon^{*2}_b} \frac{\epsilon^{*2}_b}{4}}{2c(1+\epsilon_1)(1+\epsilon_2)}} \leq \frac{\delta^*_b}{2}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent Similarly, we also have
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\label{eq:delta2}
%%	\delta_2 \leq \frac{\delta^*_b}{2}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent From Eqs. \ref{eq:delta1} and \ref{eq:delta2}, we conclude
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\label{eq:delta}
%%	\delta_1 + \delta_2 \leq \delta^*_b \leq \delta^*_a + \delta^*_b = \delta
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent The probability of Eq. \ref{eq:delta} happening is equal the probability of both Eqs. \ref{eq:given1} and \ref{eq:given2} being satisfied which is $1-\delta$. 
%	
%	Therefore, \DPIMA{} needs at most a constant times the type-2 minimum with the probability of $\Pr[\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}]$ which is at least $1-\delta$. Since we double the RR sets every round, the actual number of RR sets is at most twice the necessary one. Thus, we conclude that \DPIMA{} generates at most a constant times the type-2 minimum with probability of at least $1-\delta$.
%	
%	\begin{theorem}
%		\label{theo:dima}
%		Given a graph $G$, $0\leq \epsilon \leq 1-2/e$ and $0\leq \delta \leq 1$, let $N^2_{min}(\epsilon,\delta)$ be the type-2 minimum threshold of RR sets. 	Under \underline{reasonable assumptions}, \DPIMA{} generates no more than, to within a constant factor, $N^2_{min}(\epsilon,\delta)$ RR sets with the probability of at least $(1-\delta)$.
%	\end{theorem}
%	The Theo.~\ref{theo:dima} follows directly from Lems.~\ref{lem:epsilon_dima} and~\ref{lem:2}.
%%	\begin{proof}
%%		Given a graph $G$, $\frac{\ln\frac{2}{\delta^*_b}}{\ln \frac{1}{\delta^*_b}}\frac{4 \cdot(1+\epsilon^*_a)^2\textsf{c}_1}{(\frac{1}{2}-\frac{1}{e}-\frac{\epsilon}{2})^3}\Theta^*(\epsilon,\delta)$ RR sets, we prove that $\Pr[\delta_1 + \delta_2 \leq \delta] \geq 1-\delta$. First, we define $D$ the event that $\delta_1 + \delta_2 \leq \delta$ happens and $E$ the event that $\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}$ happens. Then,
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\Pr[A] = \Pr[A | B] \cdot \Pr[B]
%%		\end{align}
%%		\vspace{-0.2in}
%%		
%%		\noindent From Lem. \ref{lem:2}, we have
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\Pr[A | B] = \Pr[\delta_1 + \delta_2 \leq \delta | \epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}] = 1
%%		\end{align}
%%		\vspace{-0.2in}
%%		
%%		\noindent In addition, from Lem. \ref{lem:epsilon_dima},
%%		\vspace{-0.1in}
%%		\begin{align}
%%		\Pr[B] = \Pr\epsilon_1 \leq \frac{\epsilon^*_a+\epsilon^*_b/2}{1 - \epsilon^*_b/2}] = 1 - \delta
%%		\end{align}
%%		\vspace{-0.2in}
%%		
%%		\noindent Thus,
%%		\vspace{-0.1in}
%%		\begin{align}
%%			\Pr[\delta_1 + \delta_2 \leq \delta] = \Pr[A] = 1-\delta
%%		\end{align}
%%		\vspace{-0.2in}
%%		
%%		\noindent which completes the proof.
%%	\end{proof}

==> body/guarantee.tex <==
%\section{SSA Guarantee and Performance Analysis}
%\label{sec:approx}
%
%In this section, we will prove that \PIMA{} returns a $(1 - 1/e - \epsilon)$-approximate solution with at least $(1 - \delta)$-probability in Subsec.~\ref{subsec:approx}. Subsequently, \PIMA{} is shown to require no more than a constant factor of a type-1 minimum threshold of RR sets with the same probability in Subsec.~\ref{subsec:pima_rr}.
%
%\subsection{Approximation Guarantee}
%\label{subsec:approx}
%In this subsection, we will prove that \PIMA{} achieves the approximation factor of $(1 - 1/e - \epsilon)$ with at least $(1 - \delta)$-probability. The proof essentially contains two core components which are two conditions in our \RIS{} framework (Subsection~\ref{sub:ris_frame}): 1) prove that at termination \PIMA{} achieves a good approximation of the selected solution, $\hat S_k$, (Lem.~\ref{lem:com1}) and 2) the hidden optimal solution, $S^*_k$, is also well-estimated (Lem.~\ref{lem:com2}). Thus, combining these with Theo.~\ref{theo:type1} (Subsection~\ref{sub:ris_frame}) gives us the approximation factor $(1 - 1/e - \epsilon)$ stated in Theo.~\ref{theo:approx}.
%
%%For convenient uses, we denote $\epsilon_1 = \epsilon_2 = \sqrt{1 + \epsilon/2} - 1, \epsilon_3 = \epsilon/2(1 - 1/e)$ and $\Upsilon = 8c(1 - 1/e)^2 \ln \frac{1}{\delta} \frac{1}{\epsilon^2}$. Thus, $\Lambda_1 = (1+\epsilon_1)(1+\epsilon_2)\Upsilon$.
%
%The first component states the quality of the estimated influence of the returned solution, $\hat \I(\hat S_k)$, that \PIMA{} has at termination is shown in Lem.~\ref{lem:com1}.
%\begin{Lemma}
%	\label{lem:com1}
%	\PIMA{} returns a seed set, $\hat S_k$, with
%	\begin{align}
%		\Pr [\hat \I(\hat S_k) \leq (1 + \epsilon_{12})\I(\hat S_k)] \geq 1 - \delta/3
%	\end{align}
%	where $\epsilon_{12} = \epsilon_1 + \epsilon_2 + \epsilon_1\epsilon_2$.
%\end{Lemma}
%%\begin{proof}
%%	Recall that $\PIMA{}$ terminates when the selected seed set, $\hat S_k$, satisfies two conditions,
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\label{eq:con1}
%%		\Cov_{\R}(\hat S_k) \geq \Lambda_1
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent and
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\label{eq:con2}
%%	\hat \I(\hat S_k) \leq (1 + \epsilon_1)\I_c(\hat S_k)
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	From Corollary \ref{cor:check}, we have
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\label{eq:col1}
%%		\Pr[\I_c(S) \leq (1 + \epsilon_2)\I(S)] \geq 1 - \delta/3
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent Substitute $\I_c(\hat S_k)$ in Eq.~\ref{eq:col1} with that of Eq.~\ref{eq:con2},
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\Pr[\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)] \geq 1 - \delta/2
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent This completes the proof of Lem. \ref{lem:com1}.
%%	
%%\end{proof}
%The proof is presented in the appendix. Based on Lem.~\ref{lem:com1}, we prove the second component which also contains the influence estimation of the optimal solution, $S^*_k$.
%\begin{Lemma}
%	\label{lem:com2}
%	\PIMA{} terminates with
%	\begin{align}
%		\Pr [& \hat \I(S^*_k)\leq (1 - \epsilon_3)OPT_k \text{ or } \hat \I(\hat S_k) \geq (1 + \epsilon_{12})\I(\hat S_k)] \leq 2\delta/3 \nonumber
%	\end{align}
%	Thus,
%	\begin{align}
%		\label{eq:opt}
%		\Pr [& \hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k] \geq 1 - 2\delta/3
%	\end{align}
%\end{Lemma}
%%\begin{proof}
%%	To prove the lemma, we will first lower-bound the number of RR sets, $|\R|$, generated and, thus, show that $|\R| \geq \frac{\Upsilon(\epsilon_3,\delta/3) n}{OPT_k}$ with high probability and, then, apply Chernoff-Hoeffding's inequality. Recall that
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\hat \I(\hat S_k) = \frac{\Cov_{\R}(\hat S_k) n}{|\R|}
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Apply the first stopping condition, $\Cov_{\R}(\hat S_k) \geq \Lambda_1$,
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\hat \I(\hat S_k) \geq \frac{\Lambda_1 n}{|\R|} = \frac{(1 + \epsilon_1)(1 + \epsilon_2) \Upsilon(\epsilon_3,\delta/3) n}{|\R|} \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent where $\Upsilon(\epsilon_3,\delta/3) = 2c\ln (3/\delta)1/\epsilon_3^2$. 
%%	
%%	\noindent Now, combine the result of Lem.~\ref{lem:com1} with the above inequality, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\Pr[\frac{\Upsilon(\epsilon_3,\delta/3) n}{|\R|} \leq \I(\hat S_k)] \geq 1-\delta/3 \nonumber
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent Thus,
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\Pr[|\R| \geq \frac{\Upsilon(\epsilon_3,\delta/3) n}{\I(\hat S_k)}] \geq 1-\delta/3
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent and due to $\I(\hat S_k) \leq OPT_k$,
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\label{eq:num_sam}
%%	\Pr[|\R| \geq \frac{\Upsilon(\epsilon_3,\delta/3) n}{OPT_k}] \geq 1-\delta/3
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	Eq.~\ref{eq:num_sam} says that $|\R| \geq \frac{\Upsilon(\epsilon_3,\delta/3) n}{OPT_k}$ with at least $(1-\delta/3)$-probability. In cases that $|\R| \geq \frac{\Upsilon(\epsilon_3,\delta/3) n}{OPT_k}$ happens, we use Chernoff-Hoeffding's inequality (Lem. \ref{lem:chernoff}) on the optimal solution, $S^*_k$, with random variable $Z = \min\{1,|R_j \cap S^*_k|\}$ and $\mu_Z = OPT_k/n$ to obtain
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\Pr [\hat \I(S^*_k)\leq (1 - \epsilon_3)OPT_k] \leq e^{-\frac{|\R| OPT_k\epsilon^2_3}{n 2c}}
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Then, due to $|\R| \geq \frac{\Upsilon(\epsilon_3,\delta/3) n}{OPT_k}$,
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\label{eq:num_sam_sup}
%%		\Pr [\hat \I(S^*_k)\leq (1 - \epsilon_3)OPT_k] \leq e^{-\frac{\Upsilon(\epsilon_3,\delta/3)\epsilon^2_3}{2c}} = \delta/3
%%	\end{align}
%%	\vspace{-0.2in}
%%	 
%%	\noindent Thus, combining Eq.~\ref{eq:num_sam} and Eq.~\ref{eq:num_sam_sup} gives
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr [\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k] \geq 1 - 2\delta/3
%%	\end{align}
%%	\vspace{-0.2in}
%%
%%%	Accumulate the probabilities of failing when applying Lem. \ref{lem:com1} to bound the number of hyperedges and the above Chernoff-Hoeffding's inequality, we achieve
%%%	\begin{align}
%%%		\Pr [\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k] \geq 1 - \delta \nonumber
%%%	\end{align}
%%	\noindent which completes the proof of Lem. \ref{lem:com2}.
%%\end{proof}
%Lem.~\ref{lem:com1} and \ref{lem:com2} are sufficient to prove the approximation quality of \PIMA{} as stated by the following theorem.
%\begin{theorem}
%	\label{theo:approx}
%	Given $0 \leq \epsilon, \delta \leq 1$ and $\epsilon_1, \epsilon_2, \epsilon_3$ satisfying $\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2+(1-1/e)\epsilon_3 \leq \epsilon$, \PIMA{} returns a seed set, $\hat S_k$, such that,
%	\begin{align}
%		\Pr[\I(\hat S_k) \geq (1 - 1/e - \epsilon) OPT_k] \geq 1-\delta
%	\end{align}
%\end{theorem}
%
%\begin{proof} 
%	To prove the theorem, we will show that $|\R|$ is an \RIS{} threshold and then apply Theo.~\ref{theo:type1} to obtain the $(1-1/e-\epsilon)$-approximation property of \PIMA{}. Actually, we will later prove in Sec.~\ref{sec:approx} that $|\R|$ is not just \RIS{} threshold but, to within a constant factor, a type-1 minimum threshold.
%	
%	The first condition to become an \RIS{} threshold is taken from Lem.~\ref{lem:com1},
%	\begin{align}
%		\label{eq:con1_type1}
%		\Pr [\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)] \geq 1 - \delta/3
%	\end{align}
%	The second condition is obtained from Lem.~\ref{lem:com2},
%	\begin{align}
%		\label{eq:con2_type1}
%		\Pr [\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k] \geq 1 - 2\delta/3
%	\end{align}
%	\noindent From Eq.~\ref{eq:con1_type1} and Eq.~\ref{eq:con2_type1}, we conclude that $|\R|$ is an \RIS{} threshold with $\epsilon_a = (1+\epsilon_1)(1+\epsilon_2)-1$, $\epsilon_b=\epsilon_3$, $\delta_a = \delta/3$ and $\delta_b =2\delta/3$. Notice that $\epsilon_a + (1-1/e)\epsilon_b = \epsilon$ and $\delta_a + \delta_b = \delta$. By Theo.~\ref{theo:type1}, we have
%	\begin{align}
%		\Pr[\I(\hat S_k) \geq (1 - 1/e -\epsilon) OPT_k] \geq 1 - \delta
%	\end{align}
%	\noindent which completes the proof of Theo.~\ref{theo:approx}.
%%	We have bounded the number of samples. The subsequent step is to show that the optimal solution, $OPT_k$, is well-estimated.
%%	
%%	To prove the Theo. \ref{theo:approx}, we first show that probability of both $\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)$ and $\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k$ happening is at least $1 -\delta$. Let denote $\mathbb{A}$ the event that $\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)$ and $\mathbb{B}$ the event that $\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k$. Thus,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\mathbb{B} \text{ and } \mathbb{A}] = \Pr[\mathbb{B} | \mathbb{A}]\cdot \Pr[\mathbb{A}]
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent in which, $\Pr[\mathbb{A}]$ is the probability of $\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)$ happening which is proven in Lem. \ref{lem:com1} to be at least $(1-\delta/2)$ and, $\Pr[\mathbb{B} | \mathbb{A}]$ is the probability of $\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k$ happening given $\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)$ which is also proven in Lem. \ref{lem:com2} to be at least$(1-\delta/2)$. In other words, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\mathbb{A}] \geq 1-\delta/2
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent and
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\Pr[\mathbb{B} | \mathbb{A}] \geq 1-\delta/2
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	Thus,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\mathbb{B} \text{ and } \mathbb{A}] \geq (1-\delta/2)(1-\delta/2)
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent or
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\label{eq:conc}
%%		\Pr[\mathbb{B} \text{ and } \mathbb{A}] \geq 1 -\delta + \delta^2/4 \geq 1-\delta
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	At this step, we have proven that probability of both $\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)$ and $\hat \I(S^*_k)\geq (1 - \epsilon_3)OPT_k$ happening is at least $1 -\delta$. In the cases that the two events happen, we will show that \PIMA{} returns a $(1-1/e-\epsilon)$-approximate solution and, thus, conclude that \PIMA{} has that approximation factor with the probability of at least $1 -\delta$. Let $S_{kmax}$ be the size-$k$ set with maximum coverage in $\R$ when the algorithm terminates. The greedy strategy in finding max-coverage returns a set, $\hat S_k$, with $\Cov_{\R}(\hat S_k) \geq (1 - 1/e)\Cov_{\R}(S_{kmax})$ \cite{Nemhauser81} or, equivalently, $\hat \I(\hat S_k) \geq (1 - 1/e)\hat \I(S_{kmax})$. From event $\mathbb{A}$, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k) \nonumber
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent which is equivalent to
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\I(\hat S_k) \geq \hat \I(\hat S_k)- (\epsilon_1 + \epsilon_2 +\epsilon_1\epsilon_2)\I(\hat S_k) \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Since $\I(\hat S_k) \leq OPT_k$,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\I(\hat S_k) \geq \hat \I(\hat S_k)- (\epsilon_1 + \epsilon_2 +\epsilon_1\epsilon_2)OPT_k \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Apply $\hat \I(\hat S_k) \geq (1 - 1/e)\hat \I(S_{kmax})$, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\I(\hat S_k) \geq (1 - 1/e)\hat \I(S_{kmax})- (\epsilon_1 + \epsilon_2 +\epsilon_1\epsilon_2)OPT_k \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Since $S_{kmax}$ have maximum coverage, $\hat \I(S_{kmax}) \geq \hat \I(S^*_k)$ and then
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\I(\hat S_k) \geq (1 - 1/e)\hat \I(S^*_k)- (\epsilon_1 + \epsilon_2 +\epsilon_1\epsilon_2)OPT_k \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Apply event $\mathbb{B}$, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\I(\hat S_k) \geq (1 - 1/e)(1 - \epsilon_3)OPT_k- (\epsilon_1 + \epsilon_2 +\epsilon_1\epsilon_2)OPT_k \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent which is equivalent to
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\I(\hat S_k) \geq (1 - 1/e - (1 - 1/e)\epsilon_3 - \epsilon_1 - \epsilon_2 - \epsilon_1\epsilon_2)OPT_k \nonumber
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent or
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\label{eq:approx}
%%		\I(\hat S_k) \geq (1 - 1/e - \epsilon)OPT_k
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%%	\begin{align}
%%%		\I(\hat S_k) &\geq \hat \I(\hat S_k) - (\epsilon_1 + \epsilon_2+\epsilon_1\epsilon_2)\I(\hat S_k) \nonumber \\
%%%		& \geq \hat \I(\hat S_k) - (\epsilon_1 + \epsilon_2+\epsilon_1\epsilon_2)OPT_k \nonumber \\
%%%		& \geq (1 - 1/e) \hat \I(S_{kmax}) - (\epsilon_1 + \epsilon_2+\epsilon_1\epsilon_2)OPT_k \nonumber \\
%%%		& \geq (1 - 1/e) \hat \I(S^*_k) - (\epsilon_1 + \epsilon_2+\epsilon_1\epsilon_2)OPT_k \nonumber \\
%%%		& \geq (1 - 1/e) (1 - \epsilon_3)OPT_k - (\epsilon_1 + \epsilon_2+\epsilon_1\epsilon_2)OPT_k \nonumber \\
%%%		& = (1 - 1/e - (1 - 1/e)\epsilon_3 - \epsilon_1 - \epsilon_2 - \epsilon_1\epsilon_2)OPT_k \nonumber \\
%%%%		& = (1 - 1/e - \epsilon/2 - \epsilon/2)OPT_k \nonumber \\
%%%		& = (1 - 1/e - \epsilon)OPT_k \nonumber
%%%	\end{align}
%%%	Thus, 
%%%	\begin{align}
%%%	\label{eq:approx}
%%%	\I(\hat S_k) \geq (1 - 1/e - \epsilon)OPT_k
%%%	\end{align}
%%%	Note that the failure probability of Lem. \ref{lem:com2} takes into account that probability of Lem. \ref{lem:com1} and, hence, the Eq. \ref{eq:approx} holds with the same probability in Lem. \ref{lem:com2}.
%%
%%	The last inequality \ref{eq:approx} is what we want to prove and that happens with probability of both $\mathbb{A}$ and $\mathbb{B}$ happening which is at least $1-\delta$. Therefore,
%%	\begin{align}
%%		\Pr[\I(\hat S_k) \geq (1 - 1/e - \epsilon) OPT_k] \geq 1-\delta
%%	\end{align}
%\end{proof}
%
%\subsection{Achieving Type-1 Minimum Threshold}
%\label{subsec:pima_rr}
%We will analyze the number of RR sets generated in both the main and \textsf{Estimate-Inf} procedures and show that \PIMA{} requires no more than a constant times a type-1 minimum RR sets. That makes \PIMA{} the first method to achieve a type-1 minimum threshold.
%
%\textbf{Our assumptions.} The proofs in next subsection are under the two following assumptions, shall be referred as \emph{\underline{reasonable assumptions}}.
%\begin{itemize}
%\item $OPT_k \leq (1-\epsilon)|V|$. That is \emph{no $k$ nodes can influence almost all  nodes in the network}. This assumption makes the condition $\mu_Z \leq 1-\epsilon$ in Lem. \ref{lem:zo} hold. Note that this assumption can be \emph{removed} by replacing the stopping algorithm \textsf{Estimate-Inf} with the $\mathcal{AA}$ algorithm in \cite{Dagum00}.
%
%\item $\delta \leq  \frac{3}{2 \log_2 n}$. That is \emph{the error probability $\delta$ cannot be too large}. First, this assumption is compatible with the settings in the previous works. For example, in \cite{Tang14,Tang15,Nguyen16}, $\delta = 1/n$ and our assumption obviously holds since $n \gg \log_2 (n)$. In practice, frequently used values of  $\delta$  are $1\%$ or smaller. To make our assumption invalidated in those cases, $n$ will needs to exceed $2^{150} \approx 10^{45}$.
%\end{itemize}
%
%\subsubsection{Parameter Settings}
%\label{subsec:para_set}
%In Theo.~\ref{theo:approx}, we rely on the assumptions that $\epsilon_1, \epsilon_2,\epsilon_3$ are given such that,
%\begin{align}
%\label{eq:epsilon}
%\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2+(1-1/e)\epsilon_3 \leq \epsilon.
%\end{align}
%\noindent Determining their values plays an important role in the algorithm. Ideally, we want to generate just enough RR sets in the main algorithm to have a good estimate of $\hat S_k$ and then check the influence by \textsf{Estimate-Inf} procedure. That is because we will discard all the RR sets in the \textsf{Estimate-Inf} after running and, thus, if we start checking too early, we will waste a wealth of RR sets. On the other hand, because of the doubling scheme in the main algorithm, if starting checking way latter, we will generate a lot of unnecessary RR sets in the main procedure. In \PIMA{}, we determine the values of $\epsilon_1, \epsilon_2,\epsilon_3$ based on experiments and prove in next subsection that \PIMA{} generates only a constant times the type-1 threshold w.r.t these settings. In Sect.~\ref{sec:extension}, we propose a dynamic algorithm, \DPIMA{}, to tune and find the best values during the execution and it requires, within a constant factor, the strongest type-2 minimum threshold RR sets.
%
%We carried experiments on various values of $\epsilon_1,\epsilon_2$ and $\epsilon_3$ which satisfy Eq.~\ref{eq:epsilon} and found the following values robustly giving low number of RR sets,
%\begin{align}
%\label{eq:set_ep}
%\epsilon_1 & = \epsilon/6\nonumber\\
%\epsilon_2 & = \epsilon/2\\
%\epsilon_3 & = \epsilon/4(1 - 1/e) \nonumber
%\end{align}
%
%\subsubsection{Number of RR sets in the main algorithm} Here, we will analyze the number of RR sets generated in the main algorithm and show that this number is at most constant times $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ where $\epsilon_a = \epsilon_{12}=\epsilon_1 + \epsilon_2 + \epsilon_1\epsilon_2$, $\epsilon_b = \epsilon_3$ and $\delta_a = \delta/3, \delta_b = 2\delta/3$. From Subsec.~\ref{subsec:approx},
%\begin{align}
%	\label{eq:eq1}
%	\Pr [\hat \I(\hat S_k) \leq (1 + \epsilon_a)\I(\hat S_k)] \geq 1 - \delta_a
%\end{align}
%\vspace{-0.2in}
%
%\noindent and
%\vspace{-0.05in}
%\begin{align}
%	\label{eq:eq2}
%	\Pr [\hat \I(S^*_k)\geq (1 - \epsilon_b)OPT_k] \geq 1 - \delta_b
%\end{align}
%\noindent are obtained by enforcing two stopping conditions:
%\begin{align}
%	\Cov_{\R}(\hat S_k) \geq \Lambda_1 \tag{C1} \label{eq:c1}
%\end{align}
%\vspace{-0.2in}
%
%\noindent and
%\vspace{-0.05in}
%\begin{align}
%	\hat \I(\hat S_k) \leq (1 + \epsilon_1)\I_c(\hat S_k) \tag{C2} \label{eq:c2}
%\end{align}
%Now, to determine the number of RR sets generated in \PIMA{}, we will start from $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets where Eq.~\ref{eq:eq1} and Eq.~\ref{eq:eq2} are satisfied and determine how many more RR sets needed to meet (\ref{eq:c1}) and (\ref{eq:c2}). More specifically, we prove that in the cases that the inequalities in Eq.~\ref{eq:eq1} and Eq.~\ref{eq:eq2} hold with $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets, \PIMA{} needs at most $\frac{\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets, where $\textsf{c}_1$ is a constant defined in Lem.~\ref{lem:zo}. Thus, \PIMA{} will need no more than $\frac{\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets with the same probability that two inequalities in Eq.~\ref{eq:eq1} and Eq.~\ref{eq:eq2} hold which is at least $1-\delta$. The satisfaction of (\ref{eq:c1}) is stated as follows.
%
%\begin{Lemma}
%	\label{lem:num_1}
%	Suppose that with $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets, we have
%	\vspace{-0.05in}
%	\begin{align}
%		\hat \I(\hat S_k) \leq (1 + \epsilon_a)\I(\hat S_k)
%	\end{align}
%	\vspace{-0.2in}
%	
%	\noindent and
%	\begin{align}
%		\hat \I(S^*_k)\geq (1 - \epsilon_b)OPT_k
%	\end{align}
%	\noindent Then \PIMA{} needs at most $\frac{\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets to satisfy condition (\ref{eq:c1}).
%\end{Lemma}
%
%%\begin{proof}
%%	From Lem. \ref{lem:zo}, to achieve the approximation described in Eq.~\ref{eq:eq2}, we need at least $\frac{\Upsilon(\epsilon_b,\delta_b) n}{OPT_k}$ and
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\frac{\Upsilon(\epsilon_b,\delta_b) n}{OPT_k} \leq \textsf{c}_1\cdot \theta^*
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Since $\theta^*$ is the sufficient number of RR sets to achieve Eq.~\ref{eq:eq1} only and $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is enough to obtain both Eq.~\ref{eq:eq1} and Eq~\ref{eq:eq2}, we get $\theta^* \leq N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ and, thus,
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\frac{\Upsilon(\epsilon_b,\delta_b) n}{OPT_k} \leq \textsf{c}_1\cdot N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Multiply both sides by $\frac{1}{1-1/e-\epsilon}$,
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\frac{\Upsilon(\epsilon_b,\delta_b) n}{(1-1/e-\epsilon)OPT_k} \leq \frac{\textsf{c}_1\cdot N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)}{1-1/e-\epsilon}
%%	\end{align}
%%	\vspace{-0.1in}
%%	
%%	\noindent Since $\I(\hat S_k)\geq (1-1/e-\epsilon)OPT_k$ as a consequence of Eq, we have
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\label{eq:eq3}
%%		\frac{\Upsilon(\epsilon_b,\delta_b) n}{\I(\hat S_k)} \leq \frac{\textsf{c}_1\cdot N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)}{1-1/e-\epsilon}
%%	\end{align}
%%	\vspace{-0.1in}
%%	
%%	Recall that $\hat \I(\hat S_k) = \frac{\Cov_{\R}(\hat S_k)n}{|\R|}$ or $|\R| = \frac{\Cov_{\R}(\hat S_k)n}{\hat \I(\hat S_k)}$. Thus, the condition $\Cov_{\R}(\hat S_k) \geq \Lambda_1$ is equivalent to
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\label{eq:eq4}
%%		|\R| \geq \frac{\Lambda_1 n}{\hat \I(\hat S_k)} = \frac{(1+\epsilon_b)\Upsilon(\epsilon_b,\delta_b) n}{\hat \I(\hat S_k)}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent Since $\hat \I(\hat S_k) \leq (1 + \epsilon_a)\I(\hat S_k)$, we also have
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\label{eq:eq6}
%%		\frac{\Upsilon(\epsilon_b,\delta_b) n}{\I(\hat S_k)} \geq \frac{(1+\epsilon_b)\Upsilon(\epsilon_b,\delta_b) n}{\hat \I(\hat S_k)}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	From Eq.~\ref{eq:eq4} and Eq.~\ref{eq:eq6}, observe that if we set $|\R| = \frac{\Upsilon(\epsilon_b,\delta_b) n}{\I(\hat S_k)}$ then Eq.~\ref{eq:eq4} will hold and, in turn, we achieve $\Cov_{\R}(\hat S_k) \geq \Lambda_1$. Based on that and Eq.~\ref{eq:eq3}, we conclude that $\frac{\textsf{c}_1\cdot N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)}{1-1/e-\epsilon}$ RR sets are sufficient to satisfy the condition (\ref{eq:c1}).
%%%	\noindent Moreover, due to the doubling RR sets scheme in each iteration and the fact that \PIMA{} stops whenever Eq.~\ref{eq:eq4} is satisfied, we have
%%%	\vspace{-0.1in}
%%%	\begin{align}
%%%	\label{eq:eq5}
%%%	|\R| \leq 2\frac{\Upsilon_3 n}{\I(\hat S_k)}
%%%	\end{align}
%%%	\vspace{-0.2in}
%%%	
%%%	Thus, combining Eq. \ref{eq:eq3} and Eq. \ref{eq:eq5}, we get
%%%	\vspace{-0.1in}
%%%	\begin{align}
%%%	|\R| \leq \frac{2\textsf{a} }{1-1/e-\epsilon}\theta^*(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2,\epsilon_3,\delta/2,\delta/2)
%%%	\end{align}
%%%	\vspace{-0.2in}
%%\end{proof}
%
%%\noindent and we know that when the algorithm finishes,
%%\vspace{-0.05in}
%%\begin{align}
%%	\I(\hat S_k) \geq (1-1/e-\epsilon)OPT_k
%%\end{align}
%%\vspace{-0.2in}
%
%%\noindent Thus,
%%\vspace{-0.1in}
%%\begin{align}
%%\label{eq:sam}
%%	|\R| \leq \frac{2}{1-1/e-\epsilon}\frac{\Upsilon_3 n}{OPT_k}
%%\end{align}
%%\vspace{-0.15in}
%
%%In addition, apply Lem. \ref{lem:zo} where $\mu = OPT_k/n$, we have 
%%\vspace{-0.05in}
%%\begin{align}
%%\label{eq:opt_sam}
%%T=\frac{\Upsilon_3 n}{OPT_k} \leq \textsf{a}\cdot \theta^*(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2,\epsilon_3,\delta/2,\delta/2)
%%\end{align}
%%\vspace{-0.1in}
%%
%%\noindent is the sufficient number of RR sets to guarantee 
%%\vspace{-0.05in}
%%\begin{align}
%%\hat \I(S^*_k) \geq (1 - \epsilon_3)\I(S^*_k)
%%\end{align}
%%\vspace{-0.2in}
%%
%%\noindent with $(1-\delta/2)$-probability where $a$ is a constant.
%%
%%Combine Eq. \ref{eq:sam} and Eq. \ref{eq:opt_sam}, we obtain
%%\vspace{-0.05in}
%%\begin{align}
%%\label{eq:c1_sat}
%%|\R| \leq \frac{2\textsf{a}}{1-1/e-\epsilon}\theta^*(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2, \epsilon_3)
%%\end{align}
%%\vspace{-0.15in}
%
%The proof is presented in the appendix. The following lemma states that condition (\ref{eq:c2}) is also satisfied with the same number of RR sets.
%\begin{Lemma}
%	\label{lem:num_2}
%	Given all the assumptions as in Lem. \ref{lem:num_1}, \PIMA{} needs at most $\frac{\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets to satisfy condition (\ref{eq:c2}) with at least $(1-\delta/3)$-probability.
%\end{Lemma} 
%%\begin{proof}
%%	In this case, the necessary number of RR sets is the same as that to satisfy Eq.~\ref{eq:eq1} where $\epsilon_a = \epsilon_1 + \epsilon_2 + \epsilon_1\epsilon_2$. The only question here is whether the \textsf{Estimate-Inf} succeeds and returns $\I(\hat S_k)$ when the main algorithm has $|\R|$ random RR sets. Recall that it fails in the case that the number of RR sets required in \textsf{Estimate-Inf} exceeds $|\R|\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$, however, from Eq.~\ref{eq:eq3},
%%	\vspace{-0.1in}
%%	\begin{align}
%%	|\R| \geq \frac{\Upsilon(\epsilon_b,\delta_b) n}{\I(\hat S_k)} = 2c\ln \frac{3}{\delta} \frac{1}{\epsilon_3^2} \frac{n}{\I(\hat S_k)}
%%	\end{align}
%%	\vspace{-0.15in}
%%	
%%	\noindent Multiply both side with $\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$,
%%	\vspace{-0.1in}
%%	\begin{align}
%%	\label{eq:check_sam}
%%	|\R|\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2} \geq \frac{1 + \epsilon_2}{1-\epsilon_2} 2c\ln \frac{3}{\delta} \frac{1}{\epsilon_2^2} \frac{n}{\I(\hat S_k)}
%%	\end{align}
%%	\vspace{-0.1in}
%%	
%%	Based on Lem.~\ref{lem:zo}, $2c\ln \frac{3}{\delta} \frac{1}{\epsilon_2^2} \frac{n}{\I(\hat S_k)}$ random RR sets are sufficient to obtain
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\label{eq:eq11}
%%		\Pr[\I_c(\hat S_k) \geq (1-\epsilon_2) \I(\hat S_k)] \leq 1 - \delta/3
%%	\end{align}
%%	\vspace{-0.2in}
%%
%%	\noindent Thus, combine Eq.~\ref{eq:check_sam} and Eq.~\ref{eq:eq11},
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\Pr[|\R|\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2} \geq (1+\epsilon_2) 2c\ln \frac{3}{\delta} \frac{1}{\epsilon_2^2} \frac{n}{\I_c(\hat S_k)}] \leq 1 - \delta/3 \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent or,
%%	\vspace{-0.1in}
%%	\begin{align}
%%		\Pr[\frac{\I_c(\hat S_k)}{n}|\R|\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2} \geq (1+\epsilon_2) 2c\ln \frac{3}{\delta} \frac{1}{\epsilon_2^2}] \geq 1 -\delta/3 \nonumber
%%	\end{align}
%%	\vspace{-0.1in}
%%	
%%	\noindent The left hand side, $\frac{\I_c(\hat S_k)}{n}|\R|\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$, is the coverage, $\Cov$, in \textsf{Estimate-Inf} procedure when $|\R|\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$ RR sets are generated and the whole inequality is the condition to succeed. That means with $|\R|$ RR sets in the main algorithm, the \textsf{Estimate-Inf} returns a good estimation of $\I(\hat S_k)$ with at least $(1-\delta/3)$-probability.
%%\end{proof}
%
%From Lem.~\ref{lem:num_1} and Lem.~\ref{lem:num_2} and the fact that \PIMA{} stops when two stopping conditions, i.e., (\ref{eq:c1}) and (\ref{eq:c2}), are satisfied, we have the following lemma.
%%The condition (\ref{eq:c2}) is equivalent to $\hat \I(\hat S_k) \leq (1 + \epsilon_1)(1 + \epsilon_2)\I(\hat S_k)$ and is similar Eq. \ref{eq:sk} when $\epsilon_a = \epsilon_1 + \epsilon_2 + \epsilon_1\epsilon_2$. Based on Lem. \ref{lem:stop}, our stopping condition (\ref{eq:c1}) guarantees Eq. \ref{eq:sk*} with the number of samples within a constant factor from the optimal with high probability where $\epsilon_a$. The second condition (\ref{eq:c2}) is equivalent to Eq.~\ref{eq:sk}. Therefore, the number of RR sets to guarantee \ref{eq:c1} and \ref{eq:c2} is different no more than a constant factor from that to guarantee Eq. \ref{eq:sk} and \ref{eq:sk*}. Recall that \PIMA{} doubles the number of RR sets in any iteration and, hence, in the worst case, \PIMA{} generates twice the number of samples needed to satisfy the conditions \ref{eq:c1} and \ref{eq:c2}. Thus, the following lemma holds.
%\begin{Lemma}
%	\label{lem:main_proc}
%	The main algorithm of \PIMA{} generates, within a constant factor, $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets with at least $(1-\delta)$-probability.
%\end{Lemma}
%\begin{proof}
%	From Lems.~\ref{lem:num_1} and~\ref{lem:num_2}, we obtain that the number of RR sets $|\R| \geq\frac{\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is the necessary condition to satisfy both (\ref{eq:c1}) and (\ref{eq:c2}) with the probability accumulated from Eq.~\ref{eq:eq1}, Eq.~\ref{eq:eq2} and Lem.~\ref{lem:num_2} that is $1 - \delta_b -\delta/3 = 1 - \delta$ (follows from Lem.~\ref{lem:com2} that the inequalities in Eq.~\ref{eq:eq1} and~\ref{eq:eq2} are both satisfied with probability $1 - \delta_b$). Therefore, due to the doubling scheme, \PIMA{} will generate at most $\frac{2\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ which remains to be a constant times $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$.
%\end{proof}
%%
%%\textit{Remark}: Note that in fact the Condition (\ref{eq:c1}) is usually much easier to satisfy than the (\ref{eq:c2}). That is because of two reasons: 1) $\I(\hat S_k) \leq OPT_k$, so that we already need more samples to estimate $\I(\hat S_k)$ than that for $OPT_k$, 2) due to the use of \textsf{Max-Coverage} to find $\hat S_k$, the estimate $\hat \I(\hat S_k) = \Cov_{\R}(\hat S_k)$ is biased and we need more RR sets to compensate the bias. Therefore, $2N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is usually the maximum RR sets that \PIMA{} generates.
%%\begin{figure*}[!ht] \centering
%%	\includegraphics[width=0.9\linewidth]{results/examples/example2}
%%	\vspace{-0.1in}
%%	\caption{A running example of \DPIMA{}: The graph $\mathcal{G}$ is given as in the example for \PIMA{}. Additionally, \DPIMA{} only needs the precision parameters $\epsilon,\delta$. Similar to \PIMA{}, it also generates a initial collection $\mathcal{R}$ of RR sets by \RIS{} at the first step \textbf{(1)} and, then, finds \textsf{Max-Coverage} set $\hat S_k$ \textbf{(2)}. Instead of checking condition as in \PIMA{}, \DPIMA{} generates the second collection $\mathcal{R'}$ of RR sets \textbf{(3)} to obtain an estimate of $\I_{\mathcal{R}}(\hat S_k)$ and computes $\epsilon_1$ based on the two influence estimates $\I_{\mathcal{R}}(\hat S_k), \I_{\mathcal{R'}}(\hat S_k)$ \textbf{(4)}. If $\epsilon_1 \ge \epsilon$ meaning that the influence estimate $\I_{\mathcal{R}}(\hat S_k)$ is inaccurate, \DPIMA{} adds $\mathcal{R'}$ to $\mathcal{R}$ \textbf{(5)} to enrich the $\mathcal{R}$ without affecting the independence of RR sets. With the richer $\mathcal{R}$, \DPIMA{} repeats the steps \textbf{3, 4, 5} in \textbf{5, 6, 7}. It succeeds to achieve $\epsilon_1 < \epsilon$ this time. Thus, \DPIMA{} can compute $\epsilon_2,\epsilon_3,\delta_1,\delta_2$ (Lines~9-11 in Alg.~\ref{alg:dpima}) and establish the final condition $\delta_1 + \delta_2 \le \delta$.}
%%	\label{fig:exp2}
%%	\vspace{-0.1in}
%%\end{figure*}
%\subsubsection{Number of RR sets in \textsf{Estimate-Inf} procedure} As presented in Alg.~\ref{alg:check}, the number of RR sets generated in \textsf{Estimate-Inf} procedure is always smaller than $\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$ times the number of RR sets currently in the main algorithm. Therefore, the total number of RR sets generated during the running of \PIMA{} is smaller than $\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$ times the sum of RR sets present at each iteration in the main algorithm. In turn, due to the doubling behavior, the sum of RR sets is smaller than twice that number at the last iteration. Thus, based on Lem.~\ref{lem:main_proc}, we have the following lemma.
%
%\begin{Lemma}
%	\label{lem:est_proc}
%	Under \underline{reasonable assumptions}, the \textsf{Estimate-Inf} procedure of \PIMA{} generates, to within a constant factor, $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets with at least $(1-\delta)$-probability.
%\end{Lemma}
%
%%\paragraph{\textsf{Max-Coverage} procedure's Complexity.} The procedure to find \textsf{Max-Coverage} can be implemented in linear-time in terms of the total size over all the RR sets which is bounded by the number of edges examined in the generating processes. Although, \textsf{Max-Coverage} is called in all the iteration, due to the doubling behavior, the complexity of \textsf{Max-Coverage} procedure is at most twice that of generating the RR sets in the main procedure and the following lemma holds.
%
%%\begin{Lemma}
%%	\label{lem:cov_proc}
%%	The total complexity of \textsf{Max-Coverage} is at most the same as that of generating RR sets in the main algorithm.
%%\end{Lemma}
%
% Thus, we have $\ln \frac{1}{\delta_2} + \ln [2 \log_2 n] \le 2 \ln \frac{1}{\delta_2}$. The constant in the lemma is $4\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}$ times that in Lem.~\ref{lem:main_proc} that makes it,
%\begin{align}
%	4\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}\frac{2\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)
%\end{align}
%Combining Lems.~\ref{lem:main_proc} and \ref{lem:est_proc}, we conclude the overall number of RR sets by the following theorem.
%\begin{theorem}
%	\label{theo:time}
%		Under \underline{reasonable assumptions}, \PIMA{} generates, to within a constant factor, $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ RR sets with at least $(1-\delta)$-probability.
%\end{theorem}
%The total number in this theorem is the sum of those in Lems.~\ref{lem:main_proc} and \ref{lem:est_proc},
%\begin{align}
%	(1 + 4\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2})\frac{2\textsf{c}_1}{1-1/e-\epsilon}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)
%\end{align}
%%To see how strong the Theo. \ref{theo:time} is, we review the number of RR sets in the state-of-the-art methods: TIM/TIM+ prove that with their number of RR sets Eq. \ref{eq:sk} and \ref{eq:sk*} hold with $\epsilon_a=\epsilon_b=\epsilon/2$ and have no guarantee of their optimality. Since $\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2 > \epsilon/2$ and $\epsilon_3 > \epsilon/2$, we have $\theta^*(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2, \epsilon_3) < \theta^*(\epsilon/2,\epsilon/2)$. Hence, \PIMA{} requires no more than a constant times the number of RR sets in TIM/TIM+. In general, if there is an optimal method that provides good estimations for $\hat S_k$ and $S^*_k$ in form of Eq. \ref{eq:sk} and \ref{eq:sk*}, then \PIMA{} requires no more than a constant times the number of RR sets in that method with $(1 - \delta)$-probability.

==> body/ris.tex <==
%\section{Unified RIS framework}
%\label{sec:ris}
%This section presents the unified \RIS{} framework, generalizing all the previous methods of using \RIS{} sampling \cite{Borgs14,Tang14,Tang15,Nguyen16} for \IM{}. The unified framework characterizes the sufficient conditions to guarantee an $(1-1/e-\epsilon)$-approximation in the framework. Subsequently, we will introduce the concept of \RIS{} threshold in terms of the number of necessary samples to guarantee the solution quality and two types of minimum \RIS{} thresholds, i.e., type-1 and type-2.
%\subsection{Preliminaries}
%\subsubsection{RIS sampling}
%\label{subsec:ris}
%
%The major bottle-neck in the traditional methods for \IM{} \cite{Kempe03, Leskovec07, Goyal11, Nguyen2013} is the inefficiency in estimating the influence spread. To address that, Borgs et al. \cite{Borgs14} introduced a novel sampling approach for \IM{}, called Reverse Influence Sampling (in short, \RIS{}), which is the foundation for TIM/TIM+\cite{Tang14} and IMM\cite{Tang15}, the state-of-the-art methods.
%%
%%\begin{algorithm}{\RIS{} for LT model}
%%	\label{alg:ris}
%%	\begin{algorithmic}
%%		\State {\textbf{Input}: Graph $\mathcal G=(V, E, w)$.}
%%		\State {\textbf{Output}: A random RR set, $R_j \subseteq V$.}
%%		
%%		\State { 1: $R_j \leftarrow  \emptyset$}
%%		\State { 2: Pick a node $u$ with probability $\frac{b(u)}{\Gamma}$}
%%		\State { 3: \textbf{repeat}}
%%		\State { 4: \text{  \  } Attempt to select an edge $(v, u)$ using live-edge model}
%%		\State { 5: \text{  \  } \textbf{if} edge $(v, u)$ is selected \textbf{then}}
%%		\State { 6: \text{  \  \  \  \  } Set $u \leftarrow v$}
%%		\State { 7: \text{  \  \  \  \  } Add $u$ to $R_j$}
%%		\State { 8: \text{  \  } \textbf{end if}}
%%		\State { 9: \textbf{until} ($u \in R_j$) OR (no edge is selected)}
%%		\State {10: \textbf{return $R_j$}}
%%	\end{algorithmic}
%%	\vspace{-0.05in}
%%\end{algorithm}
%\begin{figure}[h!] \centering
%	\includegraphics[width=\linewidth]{results/examples/rr}
%	\caption{An example of generating random RR sets under the LT model. Three random RR sets $R_1, R_2$ and $R_3$ are generated. Node $a$ has the highest influence and is also the most frequent element across the RR sets.}
%	\label{fig:rr}
%\end{figure}
%
%Given a graph $G=(V, E, w)$, \RIS{} captures the influence landscape of $G$ through generating a set $\R$ of random \textit{Reverse Reachable (RR) sets}. The term `RR set' is also used in TIM/TIM+ \cite{Tang14,Tang15} and referred to as `hyperedge' in \cite{Borgs14}. Each RR set $R_j$ is a subset of $V$ and constructed as follows,
%\begin{Definition}[Reverse Reachable (RR) set]
%	Given $G=(V, E, w)$, a random RR set $R_j$ is generated from $G$ by 1) selecting a random node $v \in V$ 2) generating a sample graph $g$ from $G$ and 3) returning $R_j$ as the set of nodes that can reach $v$ in $g$.
%\end{Definition}
%Node $v$ in the above definition is called the \emph{source} of $R_j$. Observe that $R_j$ contains the nodes that can influence its source $v$. 
%
%If we generate multiple random RR sets, influential nodes will likely appear frequently in the RR sets. Thus a seed set $S$ that \emph{covers} most of the RR sets will likely maximize the influence spread $\I(S)$. Here a seed set $S$ covers an RR set $R_j$, if $S \cap R_j \neq \emptyset$. For convenience, we denote the coverage of set $S$ as follows,
%\begin{align}
%	\Cov_{\R}(S) = \sum_{R_j \in \R} \min\{|S \cap R_j|,1\}
%\end{align}
%
%An illustration of this intuition and how to generate RR sets is given in Fig.~\ref{fig:rr}. In the figure, three random RR sets are generated following the LT model with sources $b$, $d$ and $c$, respectively. The influence of node $a$ is the highest among all the nodes in the original graph and also is the most frequent node across the RR sets. This observation is captured in the following lemma in \cite{Borgs14}.	
%
%\begin{Lemma}[\cite{Borgs14}]
%	\label{lem:Borgs}
%	Given $G=(V, E, w)$ and a random RR set $R_j$ generated from $G$. For each seed set $S\subset V$,
%	\begin{align}
%	\I(S) = n \Pr[S \text{ covers } R_j].
%	\end{align}
%\end{Lemma}
%
%Lemma~\ref{lem:Borgs} says that the influence of a node set $S$ is proportional to the probability that $S$ intersects with a random RR set. Thus, to find $S$ that maximize $\I(S)$ can be approximated by finding $S$ that intersects as many $R_j$ as possible. The critical issue is on the minimum number of samples to provide bounded-error guarantees.
%
%\subsubsection{$(\epsilon,\delta)$-approximation}
%
%The bounded-error guarantee we seek for in our influence maximization algorithms, $(1-1/e-\epsilon)$ with probability at least $(1-\delta)$, is based on the concept of $(\epsilon, \delta)$-approximation. 
%\begin{Definition}[$(\epsilon, \delta)$-approximation]
%	Let $Z_1, Z_2,...$ be independently and identically distributed samples according to $Z$ in the interval [0, 1] with mean $\mu_Z$ and variance $\sigma_Z^2$. A \textit{Monte Carlo estimator} of $\mu_Z$,
%	\begin{align}
%	\hat \mu_Z = \frac{1}{T}\sum_{i=1}^{T}Z_i
%	\end{align}
%	is said to be an $(\epsilon, \delta)$-approximation of $\mu_Z$ if
%	\begin{align}
%	\label{eq:ed_approx}
%	\Pr [(1-\epsilon)\mu_Z \leq \hat \mu_Z \leq (1 + \epsilon) \mu_Z] \geq 1 - \delta
%	\end{align}
%\end{Definition}
%
%\noindent 
%The number of samples to guarantee an $(\epsilon, \delta)$-approximation for the Monte-Carlo method can be derived from the work of Dagum et al. \cite{Dagum00} with the proof presented in the appendix as follows,
%
%\begin{Lemma}
%	\label{lem:zo}
%	Let $\theta^*$ be the minimum number of samples that guarantee an $(\epsilon, \delta)$-approximation of $\mu_Z$ and define
%	\vspace{-0.05in}
%    \[
%    \Upsilon(\epsilon,\delta) = (2+\frac{2}{3}\epsilon) \ln (1/\delta)/\epsilon^2
%    \]
%    \vspace{-0.2in}
%    
%    and
%    \vspace{-0.1in}
%    \[
%    \Cov(Z) = \sum_{i = 1}^{T}Z_i.\] 
%    If $T = \frac{\Upsilon(\epsilon,\delta/2)}{ \mu_Z}$, then $\hat \mu_Z = \frac{\Cov(Z)}{T}$ is an $(\epsilon, \delta)$-approximate of $\mu_Z$. Further, whenever $\mu_Z \leq 1 - \epsilon$, $T$ is optimal up to a constant factor. That is
%    \vspace{-0.05in}
%	\begin{align}
%	T \leq \textsf{c}_1\cdot \theta^*
%	\end{align}
%	for some universal constant $\textsf{c}_1\geq 0$.
%\end{Lemma}
%
%The above result also extends to the case when $Z_i$ are not necessarily independent but $Cov(Z)$ satisfies \emph{martingale} properties  (see Lem. \ref{lem:chernoff} in the Appendix).
%
%%Note that calculating $T$ using the above lemma requires the knowledge of the unknown value $\mu_Z$. To avoid coping with $\mu_Z$ directly, \cite{Dagum00} also provides a simple stopping condition which depends on the number of $Z_j=1$ observed.
%%\begin{Lemma}[\cite{Dagum00}]
%%	\label{lem:stop}
%%	Let $\theta^*, \mu_Z$ be defined as in Lem.~\ref{lem:zo} and $T$ be the number of samples at which $\Cov(Z) \geq 1 + (1 + \epsilon)\Upsilon(\epsilon,\delta/2)$, then $\hat \mu_Z$ is an $(\epsilon, \delta)$-approximation of $\mu_Z$ and $T \leq (1+\epsilon)\textsf{c}_1\cdot \theta^*$ where $\textsf{c}_1$ is the constant in Lem.~\ref{lem:zo}.
%%\end{Lemma}
%%Note that if only one side of the event in Eq.~\ref{eq:ed_approx} is required, then $\Upsilon(\epsilon,\delta/2)$ becomes
%%\begin{align}
%%\label{eq:zo_side}
%%\Upsilon(\epsilon,\delta) = (2+\frac{2}{3}\epsilon) \ln \frac{1}{\delta} \frac{1}{\epsilon^2}
%%\end{align}
%
%\subsection{RIS Framework and Thresholds}
%\label{sub:ris_frame}
%Based on Lem.~\ref{lem:Borgs}, the \IM{} problem can be solved by the following two-step algorithm.
%\begin{itemize}
%	\item Generate a collection of RR sets, $\R$, from $G$.
%	\vspace{-0.05in}
%	\item Use the greedy algorithm for the Max-coverage problem \cite{Khuller1999} to find a seed set $\hat S_k$ that covers the maximum number of RR sets and return $\hat S_k$ as the solution.
%\end{itemize}
%\begin{figure}[h!] \centering
%	\vspace{-0.15in}
%	\includegraphics[width=\linewidth]{results/examples/ris_alg}
%	\caption{Overview of algorithms based on optimization over samples ($\epsilon$ is the error from approximating $f(S)$ by $\hat f_T(S)$, $OPT_f$ and $OPT_{\hat f_T}$ are optimal solutions of $f(.)$ and $\hat f_T(.)$).}
%	\label{fig:ris_alg}
%\end{figure}
%
%This two-step algorithm is actually an instance of a general class of methods illustrated in Fig.~\ref{fig:ris_alg}. The main problem of this class, in \textbf{(1)}, is an optimization problem of a function $f(.)$ over a domain $\Omega_S$. Either the function $f(.)$ is intractable to compute exactly or the problem is difficult to be tackled directly.
%
%In the first step (\textbf{(1)} to \textbf{(2)}), an approximation $\hat f_T(.)$ of $f(.)$  is constructed by generating a pool of $T = \theta(\epsilon,\delta)$ samples. Here $\theta(\epsilon,\delta)$ is an \textbf{explicit} threshold that decides the approximation quality of $\hat f_T(.)$.
%Thus the optimization problem \textbf{(1)} over $\Omega_S$ is converted to an another optimization problem of $\hat f_T(.)$ over $T$. This new optimization problem in \textbf{(2)} is expected to be more tractable than the one in \textbf{(1)}. 
%
%In the second step (\textbf{(2)} to \textbf{(3)}), an $\alpha-$approximation algorithm $\mathcal{A}$ is applied on the problem in \textbf{(2)} to find a solution $S_{\mathcal{A}}$. The solution $S_{\mathcal{A}}$ is for the function approximation $\hat f_T(.)$, however, through a dedicated bounding technique (\textbf{(3)} to \textbf{(4)}), we can show that $S_{\mathcal{A}}$ is also an approximate solution for the original problem over function $f(.)$ (\textbf{(4)} to \textbf{(1)}). Thus, the approximation guarantee for the original is accumulated from both of the steps: $\epsilon$ in function approximation and $\alpha$ in applying $\alpha$-algorithm. Thus, the overall approximation guarantee is $\alpha -\epsilon$.
%
%The optimization problem in \textbf{(1)} covers a wide range of sample-based problems, such as, targeted viral marketing \cite{Li15}, densest subgraph \cite{Bhattacharya15}, which have very high complexity to approximate and hence, need to rely on sampling algorithms. Thus, our proposed \textit{stop-and-stare} methods can be modified to address many other optimization problems under this category. 
%
%In the case of \IM{}, we apply the \textit{Stop-and-Stare} framework and propose two efficient algorithms, namely, \PIMA{} and \DPIMA{}. In context of Influence Maximization problem, the objective function $f(.)$ is the influence spread $\I(.)$ and the sample generator $T$ refers to \RIS{} sampling while the $\alpha$-approximation algorithm implies the $(1-1/e)$-greedy algorithm for the converted maximum coverage problem.
%
%As mentioned, the core issue is to determine the minimum $\theta(\epsilon,\delta)$ given a predefined setting of $\epsilon,\delta$. For \IM{}, this means \emph{``How many RR sets are sufficient to provide a good approximate solution?''}. \cite{Tang14,Tang15} propose two such theoretical thresholds and two probing techniques to realistically estimate those thresholds. However, their thresholds are not known to be any kind of minimum and the probing method is \textit{ad hoc} in \cite{Tang14} or far from the proposed threshold in \cite{Tang15}. Thus, they cannot provide any guarantee on the optimality of the number of samples generated.
%
%%Since the probing for an explicit threshold is seen to admit certain limitations, we propose a new approach. Instead of explicitly expressing a theoretical threshold and trying to probe for it, we characterize the conditions that all the \RIS{}-based algorithms need to attain and state the sufficient number of samples to satisfy those conditions. Thus, we can define the minimum samples according to the necessary conditions. We will first define our \RIS{} framework as enforcing the necessary conditions to guarantee the best known solution quality and then propose two minimum thresholds based on the precision parameters in our framework.
%
%We look into the cores of the techniques in \cite{Tang14,Tang15,Borgs14,Nguyen16} and capture the essential conditions to achieve an $(1-1/e-\epsilon)$ approximation for Influence Maximization problem. By satisfying these critical conditions, we aim to achieve a better approach rather than the prescribing a explicit threshold $\theta$ as in previous work \cite{Tang14,Tang15,Borgs14,Nguyen16}.
%
%\textbf{RIS Critical conditions.} Suppose that there is an optimal seed set $S^*_k$, which has the maximum influence in the network\footnote{If there are multiple optimal sets with influence, $OPT_k$, we choose the first one alphabetically to be $S^*_k$.}. Given $0 \leq \epsilon,\delta \leq 1$, our unified \RIS{} framework enforces two conditions:
%\begin{align}
%	\label{eq:sk}
%	\Pr[\hat \I(\hat S_k) \leq (1 + \epsilon_a) \I(\hat S_k)] \geq 1 - \delta_a
%\end{align}
%\vspace{-0.2in}
%
%\noindent and
%\vspace{-0.05in}
%\begin{align}
%	\label{eq:sk*}
%	\Pr[\hat \I(S^*_k) \geq (1 - \epsilon_b)OPT_k] \geq 1 - \delta_b
%\end{align}
%\noindent where $\delta_a + \delta_b \leq \delta\text{ and }\epsilon_a + (1-1/e)\epsilon_b \leq \epsilon$.
%
%Based on the above conditions, we define the \RIS{} threshold as the following.
%\begin{Definition}[\RIS{} Threshold]
%	\label{def:type1}
%	Given a graph $G$, $0\leq\epsilon_a, \epsilon_b, \delta_a, \delta_b\leq1$, $N(\epsilon_a, \epsilon_b, \delta_a, \delta_b)$ is called an \RIS{} Threshold in $G$ w.r.t $\epsilon_a, \epsilon_b, \delta_a, \delta_b$ if any number $|\R| \geq N(\epsilon_a, \epsilon_b, \delta_a, \delta_b)$ of random RR sets generated from $G$ is sufficient to guarantee both Eqs.~\ref{eq:sk} and~\ref{eq:sk*}.
%\end{Definition}
%%According to the above definition, if $N(\epsilon_a, \epsilon_b, \delta_a, \delta_b)$ is an \RIS{} threshold w.r.t $\epsilon_a, \epsilon_b, \delta_a, \delta_b$, any number $N \geq N(\epsilon_a, \epsilon_b, \delta_a, \delta_b)$ is also an \RIS{} threshold w.r.t $\epsilon_a, \epsilon_b, \delta_a, \delta_b$.
%Moreover, we obtain the following result connecting the two conditions as well as \RIS{} threshold with our goal of achieving $(1-1/e-\epsilon)$-approximation.
%\begin{theorem}
%	\label{theo:type1}
%	Given a graph $G$, $0\leq \epsilon_a, \epsilon_b, \delta_a, \delta_b \leq 1$, let $\epsilon \geq \epsilon_a + (1-1/e)\epsilon_b$ and $\delta \geq \delta_a + \delta_b$, if the number of RR sets $|\R| \geq N(\epsilon_a, \epsilon_b, \delta_a, \delta_b)$, then the two-step algorithm in our \RIS{} framework returns $\hat S_k$ satisfying:
%	\begin{align}
%		\Pr[\I(\hat S_k) \geq (1 - 1/e -\epsilon) OPT_k] \geq 1 - \delta
%	\end{align}
%	which means $\hat S_k$ is an $(1-1/e-\epsilon)$-approximate solution.
%\end{theorem}
%For brevity, the proof is presented in the appendix.
%%\begin{proof}
%%	According to Def.~\ref{def:type1}, if $|\R| \geq N(\epsilon_a, \epsilon_b, \delta_a, \delta_b)$ then Eqs.~\ref{eq:sk} and~\ref{eq:sk*} hold. From Eq.~\ref{eq:sk}, we have
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\hat \I(\hat S_k) \leq (1 + \epsilon_a) \I(\hat S_k)] \geq 1 - \delta_a
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent which is equivalent to
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\label{eq:5}
%%		\Pr[\I(\hat S_k) \geq \hat \I(\hat S_k) - \epsilon_a\I(\hat S_k)  ] \geq 1 - \delta_a
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	Let $S_{kmax} \in V$ be the size-$k$ set with maximum coverage in $\R$. The greedy strategy in finding max-coverage returns the set, $\hat S_k$, with $\hat \I(\hat S_k) \geq (1 - 1/e)\hat \I(S_{kmax})$ \cite{Nemhauser81}. Since $\hat \I(S_{kmax}) \geq \hat \I(S^*_k)$, $\hat \I(\hat S_k) \geq (1 - 1/e)\hat \I(S^*_k)$. Thus,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\I(\hat S_k) \geq (1 - 1/e)\hat \I(S^*_{k}) - \epsilon_a\I(\hat S_k)  ] \geq 1 - \delta_a \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Now by substituting $\hat \I(S^*_k)$ in this probability with that from Eq.~\ref{eq:sk*} and noting that the right hand side is updated to $1-\delta_a -\delta_b \geq 1-\delta$ to account for the probability in Eq.~\ref{eq:sk*}. Hence,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\I(\hat S_k) \geq (1 - 1/e)(1 - \epsilon_b)OPT_k - \epsilon_a\I(\hat S_k)  ] \geq 1 - \delta \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent Since $\I(\hat S_k) \leq OPT_k$,
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\Pr[\I(\hat S_k) \geq (1 - 1/e)(1 - \epsilon_b)OPT_k - \epsilon_aOPT_k  ] \geq 1 - \delta \nonumber
%%	\end{align}
%%	\vspace{-0.25in}
%%	
%%	\noindent or,
%%	\vspace{-0.05in}
%%	\begin{align}
%%		\Pr[\I(\hat S_k) \geq (1 - 1/e - (1 - 1/e)\epsilon_b - \epsilon_a)OPT_k  ] \geq 1 - \delta \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent and, finally, due to $\epsilon \geq \epsilon_a + (1-1/e)\epsilon_b$,
%%	\vspace{-0.05in}
%%	\begin{align}
%%	\Pr[\I(\hat S_k) \geq (1 - 1/e - \epsilon)OPT_k  ] \geq 1 - \delta \nonumber
%%	\end{align}
%%	\vspace{-0.2in}
%%	
%%	\noindent That completes the proof of Theo. \ref{theo:type1}.
%%\end{proof}
%
%\noindent \textbf{Existing \RIS{} thresholds.}
%For any $\epsilon, \delta \in (0, 1)$, Tang et al. established in \cite{Tang14} an \RIS{} threshold,
%\begin{align}
%	\label{eq:theta_1}
%	N(\frac{\epsilon}{2},\frac{\epsilon}{2},\frac{\delta}{2{n\choose k}},\frac{\delta}{2{n\choose k}}) = (8 + 2\epsilon)n \frac{ \ln 2/\delta + \ln {n \choose k} }{ \epsilon^2 OPT_k}
%\end{align}
%In a later study \cite{Tang15}, they reduced this number to another \RIS{} threshold,
%\begin{align}
%	\label{eq:theta}
%	N(\epsilon_1,\epsilon-\epsilon_1,\frac{\delta}{2{n\choose k}},\frac{\delta}{2{n\choose k}}) = 2n \frac{((1-1/e)\alpha + \beta)^2}{ \epsilon^2 OPT_k},
%\end{align}
%where $\alpha = (\ln\frac{2}{\delta})^{\frac{1}{2}}$, $\beta =~ (1-1/e)^{\frac{1}{2}}(\ln \frac{2}{\delta} + \ln \scriptsize{{n \choose k}})^{\frac{1}{2}}$ and $\epsilon_1 =\frac{\epsilon\cdot \alpha}{(1-1/e)\alpha + \beta}$. Also, based on Lemma~6 in \cite{Tang15}, we obtain another threshold with a slightly loose constant,
%\begin{align}
%	\label{eq:theta_2}
%	N = (2+\frac{2\epsilon}{3})n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{\epsilon^2 OPT_k} \leq (2+\frac{2\epsilon}{3})n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{\epsilon^2 k}
%\end{align}
%
%Unfortunately, computing $OPT_k$ is intractable, thus, the proposed algorithms have to generate $\theta \frac{OPT_k}{KPT^+}$ RR sets, where $KPT^+$ is the expected influence of a node set obtained by sampling k nodes with replacement from $G$ and the ratio $\frac{OPT_k}{KPT^+} \geq 1$ is not upper-bounded. That is they may generate many times more RR sets than needed as in \cite{Tang14}.
%%In contrast, our proposed \PIMA{} and the dynamic version, \DPIMA{} presented in Section \ref{sec:extension}, algorithms guarantee that the number of RR sets is at most a constant times the optimal number with a specific approximation requirement. We consider the class of methods that have to guarantee good approximations of the influence of the optimal and the returned seed sets. All of the previous works \cite{Borgs14,Tang14,Tang15}, which use random RR sets to capture the influence, fall under this category.
%
%%Tang et al.'s methods \cite{Tang14,Tang15} follow a general framework of using RR sets to find an $(1-1/e-\epsilon)$-approximate seed set. The framework guarantees the $(1-1/e-\epsilon)$-approximation factor as long as the influences of the selected and the optimal seed sets are estimated close enough. In other words, the following two conditions need to be fulfilled,
%%\begin{figure*}[!ht] \centering
%%	\includegraphics[width=0.9\linewidth]{results/examples/example1}
%%	\vspace{-0.1in}
%%	\caption{A running example of \PIMA{}: A graph $\mathcal{G},k=1$ and the parameters $\{\epsilon_1,\epsilon_2,\epsilon_3,\delta_1,\delta_2\}$ are given as input of \PIMA{}. The first step \textbf{(1)} is generating the first collection $\mathcal{R}$ of RR sets by \RIS{} sampling. Having generated $\mathcal{R}$, it solves the \textsf{Max-Coverage} on $\mathcal{R}$ \textbf{(2)} to find the candidate solution $\hat S_k$ and check whether $\Cov_{\mathcal{R}}(\hat S_k) \ge \Lambda_1$ (the first stopping condition). In the examples, it fails the condition. Thus, the following step \textbf{(3)} doubles the RR sets in $\mathcal{R}$ and step \textbf{(4)} solves the \textsf{Max-Coverage} \textbf{(4)} on the new $\mathcal{R}$. Eventually, the new candidate $\hat S_k$ satisfies $\Cov_{\mathcal{R}}(\hat S_k) \ge \Lambda_1$. After the satisfaction of the first condition, \PIMA{} calls an independent check \textbf{(5)} which generates an independent collection $\mathcal{R'}$ of RR sets and, then, it checks the second stopping condition that whether $\I_{\mathcal{R}}(\hat S_k) \leq (1+\epsilon_1) \I_{\mathcal{R'}}(\hat S_k)$ ($\I_{\mathcal{R}}(\hat S_k) = \hat \I(\hat S_k), \I_{\mathcal{R'}}(\hat S_k) = \I_c(\hat S_k)$ in the algorithm description). If the second condition is passed \textbf{(6)}, \PIMA{} returns the current candidate $\hat S_k$ as the solution with high confidence.}
%%	\label{fig:exp1}
%%	\vspace{-0.1in}
%%\end{figure*}
%
%\subsection{Two Types of Minimum Thresholds}
%Based on the definition of \RIS{} threshold, we now define two strong theoretical limits, i.e. type-1 minimum and type-2 minimum thresholds. In Section \ref{sec:approx}, we will prove that our first proposed algorithm, \PIMA{}, achieves, within a constant factor, a type-1 minimum threshold and later, in Section \ref{sec:extension}, our dynamic algorithm, \DPIMA{}, is shown to obtain, within a constant factor, the strongest type-2 minimum threshold.
%\begin{Definition}[type-1 minimum threshold]
%	\label{def:type1_min}
%	Given\\ $0 \leq \epsilon,\delta \leq 1$ and $0 \leq \epsilon_a,\epsilon_b,\delta_a,\delta_b \leq 1$ satisfying $\delta_a + \delta_b \leq \delta\text{ and }\epsilon_a + (1-1/e)\epsilon_b \leq \epsilon$, $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is called a type-1 minimum threshold w.r.t $\epsilon_a, \epsilon_b,\delta_a,\delta_b$ if $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is the smallest number of RR sets that satisfies both Eq.~\ref{eq:sk} and Eq.~\ref{eq:sk*}.
%\end{Definition}
%
%If $N(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is an \RIS{} threshold, then any $N$ such that $N \geq N(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ is also an \RIS{} threshold. We choose the smallest number over all such \RIS{} thresholds to be type-1 minimum as defined in Def.~\ref{def:type1_min}. All the previous methods \cite{Borgs14,Tang14,Tang15} try to approximate $N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$ for some setting of $\epsilon_a,\epsilon_b,\delta_a,\delta_b$, however, they fail to provide any guarantee on how close their numbers are to that threshold. In contrast, we show that \PIMA{} achieves, within a constant factor, a type-1 minimum threshold in Section~\ref{sec:approx}. 
%Next, we give the definition of the strongest type-2 minimum threshold which is achieved by \DPIMA{} as shown in Section~\ref{sec:extension}.
%
%%Nevertheless, we will prove that \PIMA{} needs no more than a constant times $\theta^*(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2,\epsilon_3,\delta/2,\delta/2)$ RR sets (Section \ref{sec:alg}), making \PIMA{} the first method which guarantees the $1^{st}$ level optimum of RR sets with high probability. However, the $1^{st}$ level concept is constrained by a specific setting of $(\epsilon_a,\epsilon_b,\delta_a,\delta_b)$. We thus introduce the $2^{nd}$ level optimum concept which optimizes over all the settings and our dynamic \DPIMA{} algorithm achieves that optimum (Section \ref{sec:extension}).
%
%\begin{Definition}[type-2 minimum threshold]
%	Given\\ $0 \leq \epsilon,\delta \leq 1$, $N^2_{min}(\epsilon, \delta)$ is called the type-2 minimum threshold if
%	\begin{align}
%	N^2_{min}(\epsilon,\delta) = \min_{\epsilon_a,\epsilon_b,\delta_a,\delta_b}N^1_{min}(\epsilon_a,\epsilon_b,\delta_a,\delta_b)
%	\end{align}
%	where $\epsilon_a + (1-1/e)\epsilon_b=\epsilon$ and $\delta_a + \delta_b = \delta$.
%	\label{def:type2_min}
%\end{Definition}
%From Def.~\ref{def:type2_min}, it follows that type-2 minimum is the strongest possible threshold that we can achieve in the \RIS-framework.
%
%\subsection{Achieving the Minimum Thresholds}
%In the following sections, we propose two approximation algorithms, namely, \textit{Stop-and-Stare} (\PIMA{}) and the dynamic version \DPIMA{}, which respectively achieve the two theoretical minimum thresholds as well as the best known worst-case approximation ratio. In more details, both \PIMA{} and \DPIMA{} employ the stop-and-stare strategy that doubles the number of \RIS{} samples and checks the quality of current solution by an independent influence estimation procedure. This strategy guarantees that we do not oversample, i.e., doubling the necessary number in the worst case. On a specific setting of the tuple $\{\epsilon_a,\epsilon_b,\delta_a,\delta_b\}$, \PIMA{} guarantees a type-1 minimum threshold corresponding to that configuration. 
%
%By specifically setting the parameters, \PIMA{} algorithm is simpler than the dynamic \DPIMA{}. \DPIMA{} achieves the type-2 minimum threshold through dynamically finding the best set of parameter values at each exponential checking points. Thus, $\{\epsilon_a,\epsilon_b,\delta_a,\delta_b\}$ are not specified in advance but automatically detected by \DPIMA{}. Further, \DPIMA{} can reuse the RR sets generated in the independent influence estimation without changing the independence property of RR sets in subsequent iterations.
%
%%The concept of $2^{nd}$ level optimum is the strongest form meaning that we cannot use fewer than that number of RR sets in the framework.
%
%%In the following, we will show that each component of \PIMA{} either generates no more than a constant times $\theta^*(\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2,\epsilon_3,\delta/2,\delta/2)$ with high probability or has the same complexity as the first case.
%%\CTVM{} generalizes several other viral marketing problems studied previously,
%%\begin{itemize}
%%	\item Influence Maximization (\IM): given $k \le n$, find a seed set of size $k$ that maximizes $\I(S)$. Because \IM{} assumes all nodes have the same role, by setting benefit and cost of each node to 1, we reduce \CTVM{} to \IM{}.
%%	\item Budgeted Influence Maximization (\BIM): given a budget $B$, find a seed set with total cost at most $B$, that maximizes $\I(S)$. In this case, setting benefit of each nodes to 1 will convert \CTVM{} to \BIM{}.
%%	\item Targeted Viral Marketing (\TVM): given a budget of $k \le n$ and a specific set of targeted nodes $\mathcal T$, find a seed set of size $k$ that maximizes the number of influenced nodes in $\mathcal T$. Similarly, by setting cost of each node to 1 and benefit of targeted nodes to 1, benefit of other nodes to 0 in \CTVM{}, we obtain \TVM{}.
%%\end{itemize}
%%
%%Since \IM{} is a subproblem of \CTVM{}, \CTVM{} inherits the NP-hardness property of \IM{}\cite{Kempe03}. In Table \ref{tab:syms}, we summarize all the notations used in this paper.
%
%
%%	\emph{Greedy approach}. The Greedy approach in \cite{Kempe03}, referred to as the \textsf{Greedy}, starts with an empty seed set $S = \emptyset$, and iteratively adds to $S$ a node $u$ that leads to the largest increase in the objective, i.e.,
%%	\[
%%	u = \arg \max_{v \notin S} (\I( S \cup \{v\}) - \I(S))
%%	\]
%%	The main bottle-neck is that we have to repeatedly compute $\I(S)$ to a reasonable accuracy using Monte-Carlo method. To estimate $\I(S)$, we first generate a sample graph $g$ of $\mathcal G$ using the live-edge model: select for each node $v \in \mathcal G$ at most one of its incoming edges at random, such that the edge $(u, v)$ is selected with probability $w(u, v)$, and no edge is selected with probability $1 - \sum_{u} w(u, v)$. We then measure the number of nodes reachable from $S$ in $g$, say $R_g(S)$. After generating enough sample graphs $g$ (typically $ns=10,000$ samples \cite{Kempe03}), we can take the average of $R_g(S)$ as an estimation of $\I(S)$. 
%%	
%%	To a select a node $u$, we may have to perform up to $n$ estimations of $\I(.)$ that require generating $ns$ samples each. Thus, \textsf{Greedy} with its $O(k\times ns\times m n)$ time complexity is computationally prohibitive for networks with millions of nodes. Even the recently improved heuristics CELF and CELF++ \cite{Goyal11_celf++} do not scale well for large  networks.
%
%%	In next section, we will discuss a recent sampling strategy introduced by Borgs et al. \cite{Borgs14}  for \IM{} and propose an adapted version when the node benefit is present. All the notations used in this paper are summarized in Table \ref{tab:syms}.

==> body/rois.tex <==
\subsubsection{Multi-Set Influence Estimation Oracle}
Interestingly, we can utilize our \ROS{} samples to propose a highly efficient and robust oracle to answer simultaneous influence queries. We first demonstrate the relations between \ROS{} samples and the spread influence of a set $S$ in the following lemma.
\begin{Lemma}
	\label{lem:multi_set_rois}
	Given a random \ROS{} sample $R_j$ generated from the stochastic graph $\G=(V,E,w)$, for a set $S \subseteq V$, we have the following equality,
	\begin{align}
	\label{eq:lem6}
	\I(S) = \Pr[R_j \cap S \neq \emptyset] \cdot \Gamma + \sum_{v \in S} (1-\gamma_v),
	\end{align}
	where $\Gamma = \sum_{v \in V} \gamma_v$ and $\gamma_v$ is defined in Eq.~\ref{eq:gamma_v}.
\end{Lemma}
\begin{proof}
	We start from the definition of influence spread as follows,
	\begin{align}
	\I(S) & = \sum_{v \in V} \sum_{g \in \Omega_\G} \eta_g(S,v) \Pr[g] \nonumber \\
	& = \sum_{v \in V} \Big (\sum_{g \in \Omega^\emptyset_\G(v)} \eta_g(S,v) \Pr[g] + \sum_{g \in \bar \Omega^\emptyset_\G(v)} \eta_g(S,v) \Pr[g]\Big ) \nonumber
	\end{align}
	Recall that for a node $v$, $\Omega^\emptyset_\G(v)$ contains all the sampled graphs $g$ in which $v$ has no in-coming nodes and $\bar \Omega^\emptyset_\G(v) = \Omega_\G \backslash \Omega^\emptyset_\G$. Since in each $g \in \Omega^\emptyset_\G(v)$, the node $v$ does not have any in-coming nodes, $\eta_g(S,v) = 1$ only if $v \in S$. Thus, we have $\sum_{v \in V} \sum_{g \in \Omega^\emptyset_\G(v)} \eta_g(S,v) \Pr[g] = \sum_{v \in S} \sum_{g \in \Omega^\emptyset_\G(v)} \Pr[g] = \sum_{v \in S} (1-\gamma_v)$. Combined with $\I(S)$, we obtain,
	\begin{align}
	\label{eq:lem6_eq1}
	\I(S) = \sum_{v \in V} \sum_{g \in \bar \Omega^\emptyset_\G(v)} \eta_g(S,v) \Pr[g] + \sum_{v\in S} (1-\gamma_v)
	\end{align}
	Similarly to the proof of Lemma~\ref{lem:comp_ext}, we define the graph sample space $\bar \Omega^\emptyset_\G(v)$ in which the sampled graph $\bar g \in \bar \Omega^\emptyset_\G(v)$ has a probability of $\Pr[\bar g \in \bar \Omega^\emptyset_\G(v)] = \frac{\Pr[\bar g \in \Omega_\G]}{\gamma_v}$. Then, Eq.~\ref{eq:lem6_eq1} is equivalent to,
	\begin{align}
	\I(S) & = \sum_{v \in V} \sum_{g \in \bar \Omega^\emptyset_\G(v)} \eta_g(S,v) \frac{\Pr[g]}{\gamma_v} \gamma_v + \sum_{v\in S} (1-\gamma_v) \nonumber \\
	& = \sum_{v \in V} \sum_{\bar g \in \bar \Omega^\emptyset_\G(v)} \eta_{\bar g}(S,v) \Pr[\bar g] \gamma_v + \sum_{v\in S} (1-\gamma_v) \nonumber \\
	& = \sum_{v \in V} \sum_{\bar g \in \bar \Omega^\emptyset_\G(v)} \textbf{1}_{R_j(\bar g,v) \cap S \neq \emptyset} \Pr[\bar g] \gamma_v + \sum_{v\in S} (1-\gamma_v) \nonumber \\
	& = \sum_{v \in V} \Pr[R_j(v) \cap S \neq \emptyset] \gamma_v + \sum_{v\in S} (1-\gamma_v) \nonumber \\
	& = \sum_{v \in V} \Pr[R_j(v) \cap S \neq \emptyset] \frac{\gamma_v}{\Gamma} \Gamma + \sum_{v\in S} (1-\gamma_v) \nonumber \\
	& = \sum_{v \in V} \Pr[R_j(v) \cap S \neq \emptyset] \Pr[\src(R_j) = v]\Gamma + \sum_{v\in S} (1-\gamma_v) \nonumber \\
	& = \Pr[R_j \cap S \neq \emptyset] \cdot \Gamma + \sum_{v\in S} (1-\gamma_v)
	\end{align}
	That completes the proof.
\end{proof}

Based on the results of Lemma~\ref{lem:multi_set_rois}, we can obtain an estimate of Influence Spread $\I(S)$ by first estimating $\Pr[R_j \cap S \neq \emptyset]$ which can be done using Monte-Carlo method and then plugging that to Eq.~\ref{eq:lem6} to get an influence estimate of $S$. Therefore, to build an oracle for answering influence queries, we generate a set $\R$ of \ROS{} samples in preprocessing and afterwards return $\hat \I(S)$ as an estimate of $\I(S)$,
\begin{align}
\hat \I(S) = \frac{\Cov'_\R(S)}{|\R|}\cdot \Gamma + \sum_{v \in S} (1-\gamma_v),
\end{align}
where $\Cov'_\R(S) = |\{R_j \in \R | R_j \cap S \neq \emptyset \}|$. 

\textbf{Variance Analysis.} For each a set $S$ and \ROS{} sample $R_j$, we define a random variable $Y_j$ to have value $1$ if $R_j \cap S \neq \emptyset$ and $0$ otherwise. Thus, from Lemma~\ref{lem:comp_ext}, the expectation of $Y_j$ is $\E[Y_j] = \Pr[R_j \cap S \neq \emptyset] = \frac{\I(S) - \sum_{v \in S}(1-\gamma_v)}{\Gamma}$ and the variance of $Y_j$ is calculated as follows,
\begin{align}
& \Var[Y_j] = \E[Y_j] (1 - \E[Y_j]) \nonumber \\
& = \frac{\I(S) - \sum_{v \in S}(1-\gamma_v)}{\Gamma}\big( 1- \frac{\I(S) - \sum_{v \in S}(1-\gamma_v)}{\Gamma}\big ) \nonumber \\
& = \frac{\I(S)}{n} \big ( 1-\frac{\I(S)}{n}\big)  - \frac{\sum_{v \in S}(1-\gamma_v)}{\Gamma^2}\big ( \Gamma + \sum_{1-\gamma_v}(1-\gamma_v) - \I(S)\big) \nonumber
\end{align}
Note that in the above equation, the term $\frac{\I(S)}{n} \big ( 1-\frac{\I(S)}{n}\big)$ is the variance of the random variable when \RIS{} is applied instead of \ROS{}. Thus, if $\Gamma + \sum_{1-\gamma_v}(1-\gamma_v) - \I(S) \geq 0$, then the variance of $Y_j$ will be smaller than that when \RIS{} samples are used. In fact, the $\Gamma + \sum_{1-\gamma_v}(1-\gamma_v) - \I(S) \geq 0$ commonly holds in real-world networks due to the phenomenon that most of the nodes in the network have small influences. That is for most $v \in V$, $\I(\{v\}) \ll \Gamma$, implying for most $S \subseteq V$, $\I(S) \ll \Gamma$. Therefore, using \ROS{} samples for estimating $\I(S)$ helps reduces significantly the necessary number of samples to achieve the same quality using Monte-Carlo method in typical cases of $S \subseteq V$.

\todo{What methods can be used to determine the preprocessing samples.}

%We can modify the above algorithm to estimate $I(S)$:
%Line 5: $ObservedInf \leftarrow ObservedInf + X_s + |S|$
%
%Until: $ObservedInf \geq \Lambda(1-Pr[A_{l+1}])$ - (need checking!)
%
%\begin{Lemma}
%	For any ($\epsilon$, $\delta \in (0,1)$), there exists an algorithm that gives an ($\epsilon$, $\delta$)-approximation for $I(S)$ using at most $\Theta(\frac{1}{\epsilon^2}n)$ observed influences
%\end{Lemma}

\subsection{Influence Maximization}
%\todo{Define the problem}

Our second application of outward influence is the fundamental problem of Influence Maximization (\IM{}) \cite{Domingos01,Kempe03} over a probabilistic graph. Given a graph $\G = (V,E,w)$ and a budget $k$, the problem asks for a set $S_k$ of at most $k$ nodes that has the maximum influence over all sets with size at most $k$ in the graph.
\begin{Definition}[Influence Maximization (\IM{})] Given a probabilistic graph $\G$, a budget $k$ and two parameters $\epsilon,\delta$, the \IM{} problem asks for a set $S_k$ of size at most $k$ having the maximum influence among all other sets of size at most $k$.
	\begin{equation}
	\I(S_k) = \max_{S \subseteq V, |S| \leq k} \I(S).
	\end{equation}	
\end{Definition}

We make two generic improvements that can be applied to many \IM{} methods, especially to the most efficient class of \RIS{}-based algorithms \cite{Borgs14,Tang14,Tang15,Nguyen163}. The first improvement exploits our \ROS{} samples to address a common weakness of previous \RIS{}-based method that many samples are singular. This will vastly speedup the \IM{} methods in the prevalent cases that edge weights are small. The second improvement pertains an sample-dependent bound for the optimization problem instance applied on top of the \ROS{} samples.

\subsubsection{Exploit ROIS Samples for IM}

The state-of-the-art methods \cite{Kempe03,Leskovec07,Borgs14,Tang14,Tang15,Nguyen162,Nguyen163} for \IM{} provide an $(1-1/e-\epsilon)$-approximate solution with at least $(1-\delta)$ probability. The most recent technique using Reverse Influence Sampling (\RIS) \cite{Borgs14} shows strong advantage over traditional simulation-based methods. However, even with \RIS{} sampling, they still struggle on networks with small edge influence probabilities. The main reason is that when the edge weights are very small, most of \RIS{} samples contain only their sources and become trivial since their counts are proportional to the known source selection rates, i.e. Uniform $1/n$. Thus, generating many size-1 \RIS{} samples is inefficient.

From Lemma~\ref{lem:multi_set_rois}, the influence spread of a set $S$ can be computed through the probability $\Pr[R_j \cap S \neq \emptyset]$ which in turn can be approximated using Monte-Carlo method to generate many \ROS{} samples. Let assume that we have a set of \ROS{} samples $\R = \{R_1, R_2, \dots \}$, for each $R_j$ and a node set $S$, we define a random variable,
\begin{align}
\label{eq:varz}
Z_j(S) = \textbf{1}_{R_j \cap S \neq \emptyset} \frac{\Gamma}{n} + \frac{\sum_{v \in S} (1-\gamma_v)}{n},
\end{align}
which has $\E[Z_j(S)] = \I(S)/n$. Hence, an estimate $\hat \E_\R[Z_j(S)]$ of $\E[Z_j(S)]$ based on a set of \ROS{} samples $\R$ is given by,
\begin{align}
\label{eq:compute_ez}
\hat \E_\R(S) = \frac{\Cov'_\R(S)}{|\R|} \cdot \frac{\Gamma}{n} + \frac{\sum_{v \in S}(1-\gamma_v)}{n}.
\end{align}
which provides an influence estimate $\hat \I_\R(S)$ for the set $S$,
\begin{align}
\label{eq:compute_inf}
\hat \I_\R(S) = \frac{\Cov'_\R(S)}{|\R|} \cdot \Gamma + \sum_{v \in S}(1-\gamma_v).
\end{align}
%Here, we address the aforementioned issue by proposing to use our \ROS{} samples in place of \RIS{}. Our algorithm uses a stream of \ROS{} samples $\R = \{R_1, R_2, \dots\}$. For each $R_j \in \R$, we define a corresponding random variable $$Z_j(S) = X_j(S)+ \frac{|S|}{n \cdot \gamma_0},$$ for the set $S \subseteq V$. We have,
%\begin{align}
%	\E [ Z_j(S)]  &= \E[ X_j (S)] + \frac{|S|}{n \cdot \gamma_0} =  \frac{\I_E(S) + |S|}{n \cdot \gamma_0} = \frac{1}{n \cdot \gamma_0}\I(S). \nonumber
%\end{align}

Thus, instead of optimizing over the influence function, we can equivalently find the set $S$ to maximize $\E[Z_j(S)]$. That is because if we can obtain an $\nabla$-approximate solution $\hat S$ with respect to $\E[Z_j(S)]$, $\hat S$ is also an $\nabla$-approximate solution for maximizing over influence function $\I(S)$. Moreover, using \ROS{} sampling to estimate $\E[Z_j(S)]$ is always more beneficial than using the \RIS{} for influence maximization due to the smaller variance of $Z_j(S)$ compared to that for \RIS{} samples. Smaller variance leads to less sampling requirement and, consequently, reduces computational cost.

Therefore, the framework of applying \ROS{} sampling to solve \IM{} problem contains two main steps:
\begin{itemize}
	\item[1)] Generate a sufficiently large collection of \ROS{} samples
	\item[2)] Finding the set $S_k$ that maximizes the function $\hat \I_R(S)$ and returning $S_k$ as the solution for the \IM{} instance.
\end{itemize}
There are three inherent questions related to the two steps of our framework: 1) How many \ROS{} samples are sufficiently large? 2) How to find the set $S_k$ optimizing $\hat \I_R(S)$ over \ROS{} samples? and 3) What solution guarantee can we provide on the returned solution $S_k$ for \IM?

The first question can be answered using recent methods for \RIS{} sampling: Stop-and-Stare \cite{Nguyen163}, bounding and oversampling \cite{Tang15,Tang14}. Since the function $\hat \I_R(S)$ is monotone and submodular, the naive greedy node selection scheme gives an $(1-1/e)$-solution $\hat S_k$ for the optimization problem over \ROS{} samples. Thus, we can provide a good polynomial time approximation algorithm for the second question while the overall solution guarantee of $\hat S_k$ for \IM{} problem is a combination of estimation quality in step~1 and approximation guarantee in step~2.

\subsubsection{Maximization over ROIS Samples and Sample-dependent Bounds}
We first investigate the optimization problem of finding a set $S_k$ to maximize the function $\hat \I_\R(S)$ given a set of \ROS{} samples $\R$. The function $\hat \I_\R(S)$ is monotone and submodular since it is the weighted sum of a set coverage terms $\Cov'_\R(S)$ with the same properties and a linear term $\sum_{v \in S} (1-\gamma_v)$. 
\begin{Lemma}
	Given a set of \ROS{} samples $\R$, the set function $\hat \I_\R(S)$ defined in Eq.~\ref{eq:compute_inf} is monotone and submodular.
\end{Lemma}
\begin{proof}
	Since the function $\hat \I_\R(S)$ contains two additive terms, it is sufficient to show that each of them is monotone and submodular. The second term $\sum_{v \in S}(1-\gamma_v)$ is a linear function and thus, it is monotone and submodular. For the first additive term, we see that $\frac{\Gamma}{|\R| \cdot n}$ is a constant and only need to show that $\Cov'_\R(S)$ is monotone and submodular. Given the collection of \ROS{} samples $\R$ in which $R_j \in \R$ is a list of nodes, the function $\Cov'_\R(S)$ is just the count of \ROS{} samples that intersect with the set $S$. In other words, it is equivalent to a covering function in a set system where \ROS{} samples are elements and nodes are sets. A set covers an element if the corresponding node is contained in the corresponding \ROS{} sample. It is well known that any covering function is monotone and submodular and thus, the $\Cov'_\R(S)$ has the same properties.
\end{proof}
Thus, a standard greedy scheme, which iteratively selects a node with highest marginal gain, gives a $(1-1/e)$-approximate solution $\hat S_k$, where the marginal gain of a node $v$ to a set $S$ is defined as follows,
\begin{align}
\Delta_\R(S,v) = \Cov'_\R(S \cup \{v\}) - \Cov'_\R(S)
\end{align}

Moreover, we present an sample-dependent bound for the solution quality of $\hat S_k$ based on the monotonicity and submodularity properties. This bound depends on the problem instance and can be combined with the $(1-1/e)$-bound to give a better guarantee on the solution. That results in faster termination for some algorithms that check the optimality of the current solution to stop. For example, the Stop-and-Stare framework \cite{Nguyen163} alternates between doubling the samples to find a better candidate and checking the quality of current solution with requirement to stop. Thus, with better bound, Stop-and-Stare halts earlier.

\begin{algorithm} \small
	\caption{\textsf{Greedy} with Sample-dependent Bounds}
	\label{alg:cov}
	\KwIn{\ROS{} sample set $\R$ and $k$}
	\KwOut{Candidate set $\hat S_k$, $\hat \I_\R(\hat S_k)$ and its bound $\nabla$}
	\tcp{Find the seed set}
	$\hat S_k = \emptyset$\\
	\For{$i=1:k$}{
		$\hat v \leftarrow \arg \max_{v\in V\backslash \hat S_k}\big (\frac{\Delta_\R(\hat S_k,v)}{|\R|}\Gamma + (1-\gamma_v)\big )$\\
		Add $\hat v$ to $\hat S_k$\\
	}
	\tcp{Upper bound distance to the optimal}
	$L = \emptyset; V_L = V \backslash \hat S_k$\\
	\For{$i =1:k$}{
		$\hat u \leftarrow \arg \max_{u\in V_L\backslash L}\big (\frac{\Delta_\R(\hat S_k, u)}{|\R|}\Gamma + (1-\gamma_u)\big )$\\
		Add $\hat u$ to $L$
	}
	\tcp{Compute the sample-dependent bound}
	$\hat \I_\R(\hat S_k) = \Cov'_\R(\hat S_k) \cdot \Gamma/|\R| + \sum_{v \in \hat S_k} (1-\gamma_v)$\\
	%	$U_k = \hat \I_\R(\hat S_k) + \sum_{v \in L}\big(\Delta_\R(\hat S_k, v)\cdot \Gamma/|\R| + (1-\gamma_v)\big)$\\
	$\nabla_s = \frac{\hat \I_\R(\hat S_k)}{\hat \I_\R(\hat S_k) + \sum_{v \in L}\big(\Delta_\R(\hat S_k, v)\cdot \Gamma/|\R| + (1-\gamma_v)\big)}$ \\
	%	\If{$\nabla < 1-1/e$}{$\nabla = 1-1/e$}
	%	$\nabla = \max\{\nabla, 1-1/e \}$ \\
	\textbf{return} $<$$\hat S_k, \hat \I_\R(\hat S_k), \max\{\nabla_s, 1-1/e \}$$>$
\end{algorithm}

Given a collection of \ROS{} samples $\R$ and a budget $k$, the Greedy algorithm combined with our input-dependent bound is presented in Alg.~\ref{alg:cov}. The algorithm contains two main steps:
\begin{itemize}
	\item Find the solution $\hat S_k$ via greedy strategy: iteratively selects a node with largest marginal gain (Line~3) and add to $\hat S_k$ until $k$ nodes have been selected.
	\item Compute an upper-bound the optimal solution: This bound is measured by adding the $k$ largest marginal gains to $\hat S_k$ to $\hat \I_\R(\hat S_k)$ (Line~7-8). The upper-bound is given in the denominator of Line~10 where we compute the sample-dependent bound $\nabla_s$. Since the greedy strategy guarantees that $\hat S_k$ is at least $(1-1/e)$-optimal and we obtain a sample-dependent bound $\nabla_s$, the overall approximation guarantee is the maximum between the two and gets returned.
\end{itemize}

The correctness of the upper-bound is stated in the following lemma.
\begin{Lemma}
	\label{lem:cov}
	In Alg.~\ref{alg:cov}, we have,
	\begin{align}
	\hat \I_\R(\hat S_k) + \sum_{v \in L}\big(\Delta_\R(\hat S_k, v)\cdot \Gamma/|\R| + (1-\gamma_v)\big) \geq \hat \I_\R(S_\R^*), \nonumber
	\end{align}
	where $S_\R^*$ is the optimal solution on samples $\R$.
\end{Lemma}
\begin{proof}
	Let denote $\Sigma_\R(\hat S_k, S) = \sum_{v \in S} \big(\Delta_\R(\hat S_k, v)\cdot \Gamma/|\R| + (1-\gamma_v)\big)$. From Alg.~\ref{alg:cov}, since nodes in $L$ have the maximum marginal gains, we have the following inequality,
	\begin{align}
	\label{eq:lem8_eq1}
	\Sigma_\R(\hat S_k, L) \geq \Sigma_\R(\hat S_k, S^*_\R)
	\end{align}
	By the submodularity property of $\hat \I(S)$ function,
	\begin{align}
	\hat \I_\R(\hat S_k) + \Sigma_\R(\hat S_k, S^*_\R) \geq \hat \I_\R(\hat S_k \cup S^*_k),
	\end{align}
	which implies that,
	\begin{align}
	\hat \I_\R(\hat S_k) + \Sigma_\R(\hat S_k, L) \geq \hat \I_\R(\hat S_k \cup S^*_k).
	\end{align}
	Furthermore, using the monotonicity of the function $\hat \I_\R(S)$, we also have $\hat \I_\R(\hat S_k \cup S^*_k) \geq \hat \I_\R(S^*_k)$ and thus obtain
	\begin{align}
	\hat \I_\R(\hat S_k) + \Sigma_\R(\hat S_k, L) \geq \hat \I_\R(S^*_k).
	\end{align}
	That completes the proof.
\end{proof}

The approximation guarantee of Alg.~\ref{alg:cov} is stated as follows,
\begin{Lemma}
	\label{lem:greedy}
	The Greedy algorithm with sample-dependent bound returns an $\max\{1-1/e,\nabla_s\}$-approximate solution $\hat S_k$,
	\begin{align}
	\hat \I_\R(\hat S_k) \geq \max\{1-1/e,\nabla_s\} \hat \I_\R(S^*_\R).
	\end{align}
\end{Lemma}

\subsubsection{Applications to IM Methods}

Since our \ROS{} sampling and greedy algorithm with Sample-dependent bounds are general, at this point, we can apply many optimization framework based on sampling to estimate the objective function. Specifically, a long the line of influence maximization algorithms, we can apply the two-phase method in \cite{Borgs14,Tang14,Tang15} or the most recent Stop-and-Stare framework \cite{Nguyen163}. For demonstration, we incorporate our \ROS{} sampling to the novel Stop-and-Stare framework for influence maximization. More specifically, we combine \ROS{} sampling with the \PIMA{} algorithm\footnote{\cite{Nguyen163} also proposes the dynamic \DPIMA{} algorithm, however, our sample-dependent bound cannot be applied due to the introduced dependency of our bounding technique with the dynamic computation of precision parameters. \PIMA{} has fixed precision parameters and thus, sample-dependent bound can be incorporated.} in \cite{Nguyen163} with the following modifications:
\begin{itemize}
	\item[1)] The random variable associated with each \RIS{} sample defined in \cite{Nguyen163} only ranges in $[0,1]$ but our random variable $Z_j(S)$ on \ROS{} sample takes value between $\frac{\sum_{v\in S} (1-\gamma_v)}{n}$ and $\frac{\Gamma + \sum_{v \in S}(1-\gamma_v)}{n}$. Thus, in order to bound the error and prove the approximation guarantee, we apply the generalized bound for random variable in range $[a,b]$ from Eq.~\ref{eq:gen_bound}.
	\item[2)] Our Greedy algorithm with sample-dependent bound is applied instead of the normal Maximum Coverage algorithm to find the candidate solution $\hat S_k$ in each iteration of the algorithm. Thanks to the better bound on the solution, the stopping condition in \PIMA{} can be improved. Specifically, in the original \PIMA{} algorithm, if the ratio between two influence estimations at each checking point is smaller than the threshold $\epsilon_1$, $\frac{\hat \I(\hat S_k)}{\I_c(\hat S_k)} -1 \leq \epsilon_1$ where $\epsilon_1 = \frac{\epsilon - \epsilon_3(1-1/e)-\epsilon_2}{1+\epsilon_2}$, then \PIMA{} terminates. We improve $\epsilon_1$ to $\frac{\epsilon + \nabla -1 + 1/e - \epsilon_3\nabla-\epsilon_2}{1+\epsilon_2}$ which is larger than the original $\epsilon_1$ since $\nabla \geq 1-1/e$.
	\item[3)] Recall the definition of $\Cov'_\R(S)$ as follows,
	\begin{align}
	\Cov'_{\R}(S) = |\{R_j \in \R | \R_j \cap S \neq \emptyset\}|,
	\end{align}
	and an estimate $\hat \E_\R[Z_j(S)]$ of $\E[Z_j(S)]$ based on $\R$ is
	\begin{align}
	%		\label{eq:compute_inf}
	\hat \E_\R(S) = \frac{\Cov'_\R(S)}{|\R|} \cdot \frac{\Gamma}{n} + \frac{\sum_{v \in S}(1-\gamma_v)}{n}.
	\end{align}
	which replaces the computation of $\hat \I_\R(S)$ in \PIMA{}.
\end{itemize}

Our adapted algorithm is named \OSSA{} and described in Alg.~\ref{alg:main} assuming a set of random \ROS{} samples $R^1_1, R^1_2, \dots $.

\begin{algorithm}[!h] \small
	\caption{\OSSA{} Algorithm}
	\label{alg:main}
	\KwIn{Graph $G$, a budget $k$ and precision parameters $\epsilon_1,\epsilon_2,\epsilon_3,\delta_1,\delta_2$, approximation desire $\rho$}
	\KwOut{$\Delta$-near optimal seed set $\hat S_k$ with $k$ nodes}
	%	Compute $\epsilon_1,\epsilon_2,\epsilon_3$ according to Eq.~\ref{eq:set_ep}\\
	$\Lambda \leftarrow 2 \ln(\frac{4\log_2n}{\delta_1})\frac{1}{\epsilon_3^2}$;\\
	%	$\R \leftarrow \{R^1_1, \dots, R^1_\Lambda\}$;\\
	%	\Repeat{$|\R|\geq (2+\frac{2\epsilon}{3})n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{k\epsilon^2}$}{
	\For{$i = 1:2\log_2n$}{
		$\R = \{R^1_1, \dots, R^1_{\Delta \cdot 2^i}\}$\\
		$<$$\hat S_k,\hat \I(\hat S_k), \nabla$$>\leftarrow$ \textsf{Greedy}($\R$, $k$) \tcp*{Alg.~\ref{alg:cov}}
		%		\If{$\Cov_{\R}(\hat S_k) \geq \Lambda$}{
		$\delta'_2 = \frac{\delta_2}{4\log_2n}; T_{max} = 2\frac{1 + \epsilon_2}{1-\epsilon_2}\frac{\epsilon_3^2}{\epsilon_2^2}|\R|$\\
		$\I_c(\hat S_k) \leftarrow $ \textsf{Estimate-Inf}($G, \hat S_k, \epsilon_2, \delta'_2, T_{max}$) \tcp*{Alg.~\ref{alg:check}}
		%		$\epsilon'_3 = \epsilon_3 \cdot \sqrt{\frac{n(1+\epsilon_2)}{2^i \I_c(\hat S_k)}}, $
		$\epsilon'_1 = \frac{\hat \I(\hat S_k)}{\I_c(\hat S)} - 1$;\\
		\If{$\Cov'_\R(\hat S_k) \geq (1+\epsilon'_1)(1+\epsilon_2)\Lambda \textbf{ and } \epsilon'_1 \leq \frac{(1-\epsilon_3)\nabla - \rho - \epsilon_2}{\rho + \epsilon_2}$}{
			\textbf{return} $\hat S_k$;
		}
		%		}
		%		Add to $\R$ with $R^1_{|\R|+1},\dots,R^1_{2|\R|}$;\\
	}
	\textbf{return} $\hat S_k$
\end{algorithm}

\begin{algorithm} \small
	\caption{\textsf{Estimate-Inf} procedure}
	\label{alg:check}
	\KwIn{Graph $G$, a seed set $S$, $0 \leq \epsilon_2, \delta'_2 \leq 1$ and maximum number of samples, $T_{max}$}
	\KwOut{$\I_c(S)$ such that $\I_c(S) \leq (1 + \epsilon_2)\I(S)$ with at least $(1-\delta_2)$-probability or exceeding $T_{max}$}
	$\Lambda_2 = 1+(2+\frac{2}{3}\epsilon_2)(1 + \epsilon_2)(\ln \frac{1}{\delta'_2}) \frac{1}{\epsilon_2^2}$\\
	$\Cov' = 0$\\
	\For{$j = 1:T_{max}$}{
		$\Cov' = \Cov' + \min\{|R^2_j \cap S|,1\}$\\
		\If{$\Cov' + \frac{j}{\Gamma}\sum_{v \in \hat S_k}(1-\gamma_v) \ge \Lambda_2$}{
			\textbf{return} $\I_c(S) = \frac{\Gamma}{j} \Cov'+ \sum_{v \in \hat S_k} (1-\gamma_v)$
		}
	}
	\textbf{return }0 \tcp*{Exceeding $T_{max}$ \ROS{} sets}
\end{algorithm}

In addition to the graph $\G$ and budget $k$, Alg.~\ref{alg:main} also takes $\epsilon_1,\epsilon_2,\epsilon_3,\delta_1,\delta_2$ as precision parameters which satisfy the following conditions: 
\begin{align}
\epsilon_1+\epsilon_2+\epsilon_1\epsilon_2 + \epsilon_3(1-1/e) \leq \epsilon
\\
\delta_1 + \delta_2 \leq \delta
\label{eq:delta}
\end{align}
The values of those parameters will be determined shortly. The algorithm starts by computing $\Lambda$ which is the threshold in the first stopping condition (Line~5). The main procedure is an iterative loop that uses a set of \ROS{} samples $\R$ to find the candidate solution $\hat S_k$ by the \textsf{Greedy} Algorithm~\ref{alg:cov}. If the first stopping condition is met meaning the candidate $\hat S_k$ covers enough \ROS{} samples, it will reestimate the influence of $\hat S_k$ by an independent algorithm, called \textsf{Estimate-Inf}, which is similar to Alg.~3 in \PIMA{} \cite{Nguyen163}. Afterwards, if the two estimates are close enough, i.e. within error of $\epsilon_1$, then the candidate $\hat S_k$ is returned as the final solution. $\epsilon_1$ is recalculated at every iteration when a new $\hat S_k$ is found using the sample-dependent bound $\nabla$. Otherwise, it goes to the next iteration by adding $|\R|$ more new \ROS{} samples. Similar to \PIMA{}, the guarding condition in Line~11 is only for stopping the algorithm in bad event.

\textbf{Approximation Analysis.}
The approximation quality of \OSSA{} is stated as follows:
%Our adapted algorithm is named \OSSA{} and described in Alg.~\ref{alg:dpima}.

%Thus, we can obtain an estimate of $\I(S)$ through estimating $\E[Z_j(S)]$. Thus, \OSSA{} bases on the Stop-and-Stare framework \cite{Nguyen163} to estimate $\E[Z_j(S)]$. We define $\Cov_{\R}(S)$ to be the number of \ROS{} samples $R_j \in \R$ that intersect with $S$, $R_j \cap S \neq \emptyset$,
%\begin{align}
%	\Cov_{\R}(S) = |R_j \in \R | \R_j \cap S \neq \emptyset|
%\end{align}
%and hence, an estimate of $\I(S)$ from a set $\R$ of \ROS{} samples is expressed as the following,
%\begin{align}
%	\label{eq:compute_inf}
%	\hat \I_\R(S) = \frac{\Cov_\R(S)}{|\R|} \cdot n \cdot \gamma_0 + |S|.
%\end{align}

%\todo{Analyze the variance of the new sample $\Var(Z_j) = \Var(X_j) \gamma_0^2$ }


%We combine our \ROS{} sampling with the Stop-and-Stare framework in \cite{Nguyen163} to propose an efficient and robust $(1-1/e-\epsilon)$-approximation algorithm, namely \OSSA{}. The robustness of our method is reflected by the performance consistency across different network data. In contrast, the current methods for \IM{} suffer severely in cases of having small edge influences.

%Our \OSSA{} algorithm is described in Alg.~\ref{alg:dpima}.
%
%\begin{algorithm}
%	\caption{\textsf{Max-Coverage} procedure}
%	\label{alg:cov}
%	\KwIn{\ROS{} sample set $\R$ and $k$}
%	\KwOut{Candidate set $\hat S_k$ and $\hat \I(\hat S_k)$}
%	$\hat S_k = \emptyset$\\
%	\For{$i=1:k$}{
%		$\hat v \leftarrow \arg \max_{\{v\in V\}}(\Cov_{\R}(\hat S_k\cup \{v\}) - \Cov_{\R}(\hat S_k))$\\
%		Add $\hat v$ to $\hat S_k$\\
%	}
%	\textbf{return} $<$$\hat S_k, \hat \I_\R(\hat S_k)$$>$
%\end{algorithm}
%
%\begin{algorithm}[!ht] \small
%	\caption{\OSSA{} Algorithm}
%	\label{alg:dpima}
%	\KwIn{Graph $G$, $0 \leq \epsilon, \delta \leq 1$, and $k$}
%	\KwOut{An $(1 - 1/e - \epsilon)$-optimal solution, $\hat S_k$}
%	$\Lambda \leftarrow (1 + \epsilon)^2(2+2/3\cdot \epsilon) \ln(2/\delta)\cdot 1/\epsilon^2$\\
%	$\R \leftarrow$ Generate $\Lambda$ random variables by \ROS{} sampling\\
%	\Repeat{$|\R|\geq (2+\frac{2\epsilon}{3})n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{k\epsilon^2}$}{
%		$<$$\hat S_k,\hat \I_\R(\hat S_k), \nabla$$>\leftarrow$ \textsf{Greedy}($\R,k$)\\
%		$\R' \leftarrow$ Generate $|\R|$ new random variables by \ROS{}\\
%		Compute $\hat \I_{\R'}(\hat S_k)$ and the confidence level $\delta'$ of the current candidate solution $\hat S_k$\\
%		\If{$\delta' \leq \delta$}{
%			\textbf{break}\\
%		}
%%		$\epsilon_1 \leftarrow \hat \I(\hat S_k)/\I_{c}(\hat S_k) - 1$\\
%%		\If{$(\epsilon_1 \leq \epsilon)$}{
%%			$\epsilon_2 \leftarrow \frac{\epsilon-\epsilon_1}{2(1+\epsilon_1)}$, $\epsilon_3 \leftarrow \frac{\epsilon-\epsilon_1}{2(1-1/e)}$\\
%%			$\delta_1 \leftarrow e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{(2+2/3\epsilon_3)(1+\epsilon_1)(1+\epsilon_2)}}$\\
%%			$\delta_2 \leftarrow e^{-\frac{(\Cov_{\R'}(\hat S_k)-1)\cdot \epsilon_2^2}{(2+2/3\epsilon_2)(1+\epsilon_2)} + \ln [2 \log_2 n]}$\\
%%			\If{$\delta_1+\delta_2\leq \delta$}{
%%				\textbf{return} $\hat S_k$
%%			}
%%		}
%		Merge $\R \leftarrow \R \cup \R'$ \\
%	}
%	\textbf{return} $\hat S_k$
%\end{algorithm}
%
%\OSSA{} iteratively generates two same-size independent sets of \ROS{} samples, $\R$ and $\R'$. $\R$ helps find the candidate solution $\hat S_k$ and $\R'$ verifies whether $\hat S_k$ satisfies the quality requirement declared by $\epsilon,\delta$. It first generates $\R$ with the first $\Upsilon$ samples (Line~1-2) which is the minimum number to fulfill the stopping condition (Line~7). Our \textsf{Greedy} algorithm with sample-dependent bound (Alg.~\ref{alg:cov}) is applied on $\R$ to find the candidate solution $\hat S_k$ that covers at least $\nabla$ the optimal, $\Cov_\R(\hat S_k) \geq \nabla \max_{|S| \leq k} \Cov_\R(S)$. Afterward, the algorithm generates the second set $\R'$ of samples and obtain another estimate $\I_{\R'}(S)$ to compute the confidence level $\delta'$,
%\begin{align} \small
%	&\delta' = \delta_1 + \delta_2 \nonumber \\
%	&\delta_1 \leftarrow e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{(2+2/3\epsilon_3)(1+\epsilon_1)(1+\epsilon_2)}}, \delta_2 \leftarrow e^{-\frac{(\Cov_{\R'}(\hat S_k)-1)\cdot \epsilon_2^2}{(2+2/3\epsilon_2)(1+\epsilon_2)} + \ln [2 \log_2 n]} \nonumber \\
%	&\epsilon_1 \leftarrow \hat \I_\R(\hat S_k)/\hat \I_{\R'}(\hat S_k) - 1, \epsilon_2 = \epsilon_3 \leftarrow \frac{\nabla-(1-1/e) + \epsilon - \epsilon_1}{1+\epsilon_1 + \nabla} \nonumber	
%\end{align}
%If the confidence level $\delta'$ dominates $\delta$, $\delta' \leq \delta$, we conclude that $\hat S_k$ is an $(1-1/e-\epsilon)$-approximate solution with probability of at least $(1-\delta)$.

%From Theorem~5 in \cite{Nguyen163}, we obtain results for \OSSA{}.

\begin{theorem}
	\label{theo:ossa}
	Given a graph $\G = (V,E,w)$, budget $k$, a desired approximation factor requirement $\rho \leq 1-1/e-\epsilon$ and precision parameters $\epsilon_1, \epsilon_2, \epsilon_3,\delta_1,\delta_2$, \OSSA{} returns an $\rho$-approximate solution with a probability of at least $(1-\delta)$ where $\delta = \delta_1 + \delta_2$.
	%	The number of \ROS{} samples generated in \OSSA{} is optimal in the Stop-and-Stare framework.
\end{theorem}
To prove this theorem, we will show that at any particular iteration with $i = 1, \dots, 2 \log_2(n)$ and $\Delta\cdot 2^i$ \ROS{} samples, the candidate solution $\hat S_k$ achieves a level of quality guarantee. \OSSA{} terminates when the achieved guarantee satisfies the given precision requirement specified by $\epsilon_1, \epsilon_2, \epsilon_3, \delta_1, \delta_2$.

We first establish the following lemma about the estimation quality of the \textsf{Estimate-Inf} procedure.
\begin{Lemma}
	\label{lem:est_inf}
	Given $\epsilon_2, \delta'_2$, the \textsf{Estimate-Inf} algorithm returns an estimate $\I_c(S)$ of $\I(S)$ that,
	\begin{align}
	\Pr[\I_c(S) \leq (1+\epsilon_2) \I(S)] \geq 1 - \delta'_2 = 1-\frac{\delta_2}{4 \log_2(n)}.
	\end{align}
\end{Lemma}
Since \textsf{Estimate-Inf} is special case of our Generalized Stopping Rule Alg. when $\alpha = 1$ and Lemma~\ref{lem:est_inf} follows directly from Theorem~\ref{theo:stop}.

Let consider a particular iteration $i$ of the loop in Alg.~\ref{alg:main} with $\Lambda\cdot 2^i$ \ROS{} samples. Assume that $S^*_k$ is the optimal solution of the \IM{} instance with the corresponding influence value of $\OPT_k$, we obtain the following theorem regarding the estimation quality of $S^*_k$ using $\Lambda\cdot 2^i$ \ROS{} samples.
\begin{Lemma}
	\label{lem:opt_est}
	In iteration $i$ of Alg.~\ref{alg:main}, the optimal solution $S^*_k$ satisfies the following inequality,
	\begin{align}
	\Pr[\hat \I(S^*_k) \geq (1-\epsilon'_3) \OPT_k] \geq 1-\frac{\delta_1}{4 \log_2n},
	\end{align}
	where $\epsilon'_3 = \epsilon_3 \cdot \sqrt{\frac{n(1+\epsilon_2)}{2^i \I_c(\hat S_k)}}$.
\end{Lemma}
\begin{proof}
	Since at iteration $i$, we have a fixed number of $\Lambda\cdot 2^i$ \ROS{} samples and a well-defined $\epsilon'_3$. Apply Chernoff's bound on the approximation of $\OPT_k$ using the set of \ROS{} samples, we obtain the following,
	\begin{align}
	\Pr[\hat \I(S^*_k) \leq (1-\epsilon'_3) \OPT_k] \leq \exp(-\frac{\Lambda \cdot 2^i \OPT_k \epsilon'^2_3}{2 n})
	\end{align}
	Substituting $\Lambda$ and $\epsilon'_3$ by their definitions gives,
	\begin{align}
	\Pr[\hat \I(S^*_k) \leq (1-\epsilon'_3) \OPT_k] \leq \exp\Big(-\frac{\OPT_k(1+\epsilon_2)}{\I_c(\hat S_k)} \ln(\frac{4\log_2n}{\delta_1}) \Big) \nonumber
	\end{align}
	From Lemma~\ref{lem:est_inf}, we have that $\I(\hat S_k) \geq \frac{\I_c(\hat S_k)}{1+\epsilon_2}$ w.h.p. and know that $\I(\hat S_k) \leq \OPT_k$. Thus, we achieve that $\OPT_k \geq \frac{\I_c(\hat S_k)}{1+\epsilon_2}$ w.h.p. and then,
	\begin{align}
	\Pr[\hat \I(S^*_k) \leq (1-\epsilon'_3) \OPT_k] & \leq \exp\Big(-\ln(\frac{4\log_2n}{\delta_1})\Big) \\
	& \leq \frac{\delta_1}{4\log_2n}
	\end{align}
	which is equivalent to what we need to prove.
\end{proof}

Combine the results in Lemmas~\ref{lem:est_inf},~\ref{lem:opt_est} and guarantee of \textsf{Greedy} algorithm in Lemma~\ref{lem:greedy}, we are able to prove Theorem~\ref{theo:ossa} as follows.

\begin{proof}[of Theorem~\ref{theo:ossa}]
	Notice that in Lemma~\ref{lem:cov}, $S^*_\R$ is the optimal solution over the set $\R$ of \ROS{} samples while $S^*_k$ is the optimal solution of the \IM{} problem and hence, $\hat \I(S^*_k) \leq \hat \I(S^*_\R)$. Combine this with Lemma~\ref{lem:greedy} and Lemma~\ref{lem:opt_est}, we obtain,
	\begin{align}
		\hat \I(\hat S_k) \geq \nabla \hat \I(S^*_k),
	\end{align}
	and
	\begin{align}
		\label{eq:theo_1}
		\Pr[\hat \I(\hat S_k) \geq (1-\epsilon'_3) \nabla \OPT_k] \geq 1 - \frac{\delta_1}{4 \log_2 n}.
	\end{align}
	
	On the other hand, from Lemma~\ref{lem:est_inf} and the fact that $\hat \I(\hat S_k) = (1+\epsilon'_1) \I_c(\hat S_k)$, we have,
	\begin{align}
		\Pr[\frac{\hat \I(\hat S_k)}{1+\epsilon'_1} \leq (1+\epsilon_2) \I(\hat S_k)] \geq 1-\frac{\delta_2}{4 \log_2n},
	\end{align}
	or,
	\begin{align}
		\Pr[\frac{\hat \I(\hat S_k)}{1+\epsilon'_1} \leq \I(\hat S_k) + \epsilon_2 \I(\hat S_k)] \geq 1-\frac{\delta_2}{4 \log_2n}.
	\end{align}
	Since $\I(\hat S_k) \leq \OPT_k$, it implies that
	\begin{align}
		\Pr[\I(\hat S_k) \geq \frac{\hat \I(\hat S_k)}{1+\epsilon'_1} - \epsilon_2 \OPT_k ] \geq 1-\frac{\delta_2}{4 \log_2n}, \nonumber
	\end{align}
	
	Combine the above inequality with Eq.~\ref{eq:theo_1} and by union bound, we obtain,
	\begin{align}
		\label{eq:theo_2}
		\Pr[\I(\hat S_k) \geq (\frac{(1-\epsilon'_3)\nabla}{1+\epsilon'_1} - \epsilon_2) \OPT_k] \geq 1 - \frac{\delta_1 + \delta_2}{4 \log_2n}
	\end{align}
	Thus, at every iteration, Eq.~\ref{eq:theo_2} holds with a probability of at least  $1-\frac{\delta_1 + \delta_2}{4 \log_2n} \geq 1 - \frac{\delta}{4 \log_2 n}$. Then, by union bound, the probability that Eq.~\ref{eq:theo_2} holds at every iteration is bounded below by $1-\frac{\delta}{2}$ since there are at most $2\log_2 n$ iterations.
	
	Since at every iteration Eq.~\ref{eq:theo_2} holds with high probability, we will analyze the stopping condition in Line~8-9 to show that when the algorithm terminates, the solution $\hat S_k$ achieves the desired approximation $\rho$. The first condition $\Cov'_\R(\hat S_k) \geq (1+\epsilon'_1)(1+\epsilon_2)\Lambda$ combined with $\hat \I(\hat S_k) = (1+\epsilon'_1)\I_c(\hat S_k)$ implies that,
	\begin{align}
		(1+\epsilon'_1) \I_c(\hat S_k) \geq (1+\epsilon'_1)(1+\epsilon_2)\frac{\Lambda n}{|\R|}
	\end{align}
	Since in each iteration, we also have $|\R| = 2^i \Lambda$, it derives,
	\begin{align}
		\I_c(\hat S_k) \geq (1+\epsilon_2)\frac{n}{2^i} \Leftrightarrow \frac{(1+\epsilon_2) n}{\I_c(\hat S_k) 2^i} \leq 1
	\end{align}
	Thus, the value of $\epsilon'_3$ in Lemma~\ref{lem:opt_est} satisfies,
	\begin{align}
		\epsilon_3' \leq \epsilon_3
	\end{align}
	and the approximation guarantee from Eq.~\ref{eq:theo_2} becomes,
	\begin{align}
		\frac{(1-\epsilon'_3)\nabla}{1+\epsilon'_1} - \epsilon_2 \geq \frac{(1-\epsilon_3)\nabla}{1+\epsilon'_1} - \epsilon_2
	\end{align}
	Consider the second stopping condition of $\epsilon'_1 \leq \frac{(1-\epsilon_3)\nabla - \rho - \epsilon_2}{\rho + \epsilon_2}$, we obtain a lower bound of the approximation guarantee,
	\begin{align}
		\frac{(1-\epsilon'_3)\nabla}{1+\epsilon'_1} - \epsilon_2 \geq \frac{(1-\epsilon_3)\nabla}{1+\epsilon'_1} - \epsilon_2 \geq \rho
	\end{align}
	
	The last consideration is that whether $i$ running up to $2 \log n$ is enough to guarantee the approximation algorithm. This can be derived from \PIMA{} in \cite{Nguyen163} by observing that \PIMA{} generates at most $(2 + \frac{2}{3} \epsilon)n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{\epsilon^2}$ samples and guarantees an $1-1/e-\epsilon \geq \rho$ approximate solution with probability at least $1-\delta$. In \OSSA{}, the number of \ROS{} samples in the last iteration is $\Lambda 2^{2 \log_2 n} = 4 \ln (\frac{4 \log_2 n}{\delta_1}) \frac{1}{\epsilon_3^2} n^2 \gg (2 + \frac{2}{3} \epsilon)n \frac{\ln \frac{4}{\delta}+\ln {n\choose k}}{\epsilon^2}$ which guarantees $\hat S_k$ is an $(1-1/e-\epsilon)$ with at least $1-\frac{\delta}{2}$ probability.
	
	Thus, union bound over the probability of returning an $\rho$-approximate solution within $2 \log_2 n$ iterations and after such number of iterations, we obtain the $1-\delta$ probability of achieving the required approximation factor.
\end{proof}

\textbf{Optimal Sampling Requirement.} Observe that by setting $\rho = 1-1/e-\epsilon$ and taking the lower bound $\nabla = 1-1/e$, \OSSA{} reduces to \PIMA{} algorithm in \cite{Nguyen163} which also guarantees a type-1 optimal number of samples generated. Thus \OSSA{} algorithm guarantees a similar type-1 optimal number of samples.

\textbf{Precision Parameter Tuning.} Instead of a fixed setting of precision parameters as \PIMA{}, we propose a heuristic approach which partially relies on \OSSA{} to determine the best values of $\epsilon_1, \epsilon_2, \epsilon_3, \delta_1, \delta_2$. The algorithm is described in Alg.~\ref{alg:para_tune} assuming a set of \ROS{} samples $\R^2_1,R^2_2,\dots$.
\begin{algorithm}[!ht] \small
	\caption{Precision Parameter Tuning Algorithm}
	\label{alg:para_tune}
	\KwIn{Graph $G$, $0 \leq \epsilon, \delta \leq 1, k, \delta_1, \delta_2$ and $\rho$}
	\KwOut{Precision parameters $\epsilon_1,\epsilon_2,\epsilon_3$}
	$\Lambda' \leftarrow 2 \ln(\frac{4 \log_2n}{\delta_1})\cdot 1/\epsilon^2$\\
	%	$\R \leftarrow \{R^2_1,\dots,R^2_{\Lambda'}\}$\\
	%	\Repeat{$|\R|\geq (2+\frac{2\epsilon}{3})n \frac{\ln \frac{2}{\delta}+\ln {n\choose k}}{k\epsilon^2}$}{
	\For{$i = 1:2\log_2n$}{
		$\R \leftarrow \{R^2_1,\dots,R^2_{\Lambda'\cdot 2^i}\}$\\
		$<$$\hat S_k,\hat \I_\R(\hat S_k), \nabla$$>\leftarrow$ \textsf{Greedy}($\R,k$)\\
		$\R' \leftarrow \{R^2_{\Lambda' 2^i+1}, \dots, R^2_{\Lambda' 2^{i+1}}\}$\\
		$\epsilon_1 \leftarrow \hat \I_\R(\hat S_k)/\hat \I_{\R'}(\hat S_k) - 1$\\
		$\epsilon_2 \leftarrow \sqrt{\frac{(2+\frac{2}{3}\epsilon)(1+\epsilon)\ln\frac{4 \log_2n}{\delta_2}}{\Cov_\R'(\hat S_k)-1}}, \epsilon_3 = \sqrt{\frac{2 \ln \frac{4 \log_2n}{\delta_1}}{\Cov_\R(\hat S_k)}}$\\
%		$\delta_1 \leftarrow e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{(2+2/3\epsilon_3)(1+\epsilon_1)(1+\epsilon_2)}+ \ln [2 \log_2 n]}$\\
%		$\delta_2 \leftarrow e^{-\frac{(\Cov_{\R'}(\hat S_k)-1)\cdot \epsilon_2^2}{(2+2/3\epsilon_2)(1+\epsilon_2)} + \ln [2 \log_2 n]}$\\
		\If{$\frac{(1-\epsilon_3) \nabla}{1+\epsilon_1} - \epsilon_2 \geq \rho$}{
			\textbf{break}\\
		}
		%		$\epsilon_1 \leftarrow \hat \I(\hat S_k)/\I_{c}(\hat S_k) - 1$\\
		%		\If{$(\epsilon_1 \leq \epsilon)$}{
		%			$\epsilon_2 \leftarrow \frac{\epsilon-\epsilon_1}{2(1+\epsilon_1)}$, $\epsilon_3 \leftarrow \frac{\epsilon-\epsilon_1}{2(1-1/e)}$\\
		%			$\delta_1 \leftarrow e^{-\frac{\Cov_{\R}(\hat S_k)\cdot \epsilon_3^2}{(2+2/3\epsilon_3)(1+\epsilon_1)(1+\epsilon_2)}}$\\
		%			$\delta_2 \leftarrow e^{-\frac{(\Cov_{\R'}(\hat S_k)-1)\cdot \epsilon_2^2}{(2+2/3\epsilon_2)(1+\epsilon_2)} + \ln [2 \log_2 n]}$\\
		%			\If{$\delta_1+\delta_2\leq \delta$}{
		%				\textbf{return} $\hat S_k$
		%			}
		%		}
		%		Merge $\R \leftarrow \R \cup \R'$ \\
	}
	\textbf{return} $\hat S_k$
\end{algorithm}

The intuition behind Alg.~\ref{alg:para_tune} is that we mimic the behavior of \OSSA{} by having two set of \ROS{} samples, namely $\R$ and $\R'$, with the same cardinality. Each set provides an estimation of the seed set $\hat S_k$ which is selected by the same \textsf{Greedy} algorithm in Alg.~\ref{alg:cov}. Since, $\epsilon_1$ measures the gap between two estimations in \OSSA{}, a good estimate of $\epsilon_1$ is given in Line~6. $\epsilon_2$ and $\epsilon_3$ are assumed to have similar role and based on the condition in Eq.~\ref{eq:delta}, we compute their values accordingly. Consequently, $\delta_1$ and $\delta_2$ are related to $\Lambda$ and the \textsf{Estimate-Inf} procedure which decide the stopping condition in \OSSA{}. Thus, the algorithm stops when the accumulated probability satisfies the requirement (Line~9). Otherwise, it iterates similarly to \OSSA{}.

\textbf{Comparison to SSA}. First, due to application of the \ROS{} sampling with smaller variance implying better concentration of the generated samples, \OSSA{} needs less sampling requirement. Secondly, our sample-dependent bound of our greedy algorithm helps improve the computation of stopping criterion and stop \OSSA{} earlier than \PIMA{}. Experimentally, \OSSA{} improves \PIMA{} by a factor of an order of magnitude and surpasses all the \IM{} algorithms with the same rigorous guarantee in different edge weight models.

%\subsubsection{A Practical Bound for Maximum Coverage}

%The proof of Theorem~\ref{theo:ossa} is similar to that of Theorem~4 and 5 in \cite{Nguyen163} with one exception: Since the random variable $Z_j(S)$ ranges between $k/\gamma_0$ and $1 + k/\gamma_0$, we use the generalized bound for Martingale in Eq.~\ref{eq:gen_bound} instead of the one for $[0-1]$-random variable in \cite{Nguyen163}.

%
%\subsection{Sketch-based Influence Estimation}
%This section presents our efficient algorithm for estimating outward influence. We incorporate the optimal Monte-Carlo estimation \cite{Dagum00} with a more efficient variant of the \RIS{} sampling \cite{Borgs14}, which only generates useful non-empty samples.


==> body/sketching.tex <==
\subsection{Outward Influence Sketching}
%\todo{State the goal: Sketch to estimate influence of different seed set}

In many problems, we may need to estimate the outward influences of more than one seed sets or even all possible sets in certain size. However, the estimation based on cascade simulations can only be used for a single set. Previous work \cite{Borgs14,Tang14,Tang15,Nguyen163} proposed \textit{Reverse Influence Sampling} (\RIS{}) to sample reverse influence samples which can be used to estimate influences of many sets. Following similar idea, we introduce the \textit{Reverse Outward Influence Sampling}, denoted by \ROS{}, which serves as a building block of an oracle for querying outward influence estimates of different seed sets.

\subsubsection{RIS review}
Essentially, a random \RIS{} sample, denoted by $Q_j$, contains a \textit{randomly generated} set of nodes, following a diffusion model, that can influence a \textit{randomly selected} node, denoted by $\src(Q_j)$. A \RIS{} sample is generated in three steps:
\begin{itemize}
	\item[1)] Select a random node $v \in V$ which serves as $\src(Q_j)$.
	\item[2)] Generate a sample graph $g \sim \mathcal{G}$.
	\item[3)] Return the set $Q_j$ of nodes that can reach $v$ in $g$.
\end{itemize}
The key property of \RIS{} for estimating the influence is that the probability of a random \RIS{} intersecting with the set $S$ is proportional to $S$ influence. The formal statement is described in the following lemma.
\begin{Lemma}[\cite{Borgs14}]
	\label{lam:borgs14}
	Given a random \RIS{} sample  $Q_j$ generated from a stochastic graph $\mathcal{G} = (V,E,w)$, for a set $S \subseteq V$ of nodes, the following equality holds,
	\begin{align}
	\I(S) = n \cdot \Pr[Q_j \cap S \neq \emptyset].
	\end{align}
\end{Lemma}
Thus, to estimate the influence, we can equivalently find an estimation of $\Pr[Q_j \cap S \neq \emptyset]$. The later can be empirically done by generating multiple \RIS{} samples and taking the average over the indicator function of whether $Q_j \cap S \neq \emptyset$.

\textbf{Using RIS samples to estimate Outward Influence.} Similar to Lemma~\ref{lam:borgs14}, we establish the following relation between a \RIS{} sample and outward influence of a set $S$,
\begin{align}
\I_E(S) = n \cdot \Pr[Q_j \cap S \neq \emptyset \wedge \src(Q_j) \notin S]
\end{align}
Thus, we can estimate the outward influence by estimating the probability $\Pr[Q_j \cap S \neq \emptyset \wedge \src(Q_j) \notin S]$ that can be done by generating many \RIS{} samples $Q_j$ and taking the average of $\textbf{1}_{Q_j \cap S \neq \emptyset \wedge \src(Q_j) \notin S}$. However, a serious pitfall of this strategy is the abundant \textit{Singular Samples}, i.e. \RIS{} samples of size 1, $Q_j = \{\src(Q_j)\}$. Those singular \RIS{} samples are wasted since $\textbf{1}_{Q_j \cap S \neq \emptyset \wedge \src(Q_j) \notin S} = 0$. Unfortunately, the cases of having many singular \RIS{} samples are abundant in real-world networks where most edges have small weights, i.e. having small influences to their neighbors. Thus, this method renders severe performance inefficiency. We thus propose an efficient sampling scheme, called Reverse Outward Influence Sampling (\ROS{}), to address this issue.

\subsubsection{ROIS Sampling} 
Our procedure for generating \ROS{} consists of two major differences compared to \RIS{} sampling: 
\begin{itemize}
	\item[1)] The $\src(Q_j) = v$ is selected by an \textit{importance sampling} procedure. The importance sampling selects node $v$ proportional to the probability that a random $R_j$ from $v$ has at least one more node $u \neq v$ in addition to the $\src(R_j) = v$. That is at least one edge $(u,v)$ being realized in the sampled graph $g \sim \G$. Let denote 
	\begin{align}
	\label{eq:gamma_v}
	\gamma_v = 1-\Pi_{u \in N^{in}(v)(1-w(u,v))}.
	\end{align}
	Thus, the probability of selecting node $v$ as the $\src(R_j)$ of a random \RIS{} is computed as follows,
	\begin{align}
	\label{eq:probu}
	\Scale[1.05]{\Pr[\src(R_j) = v] = \frac{\gamma_v}{\sum_{u \in V}. \gamma_u}}.
	\end{align}
	\item[2)] From the $\src(R_j)$, we select at least one incoming node that influences $\src(R_j)$ with probability of selecting $u$,
	\begin{align}
	\label{eq:probn}
	\Pr[\text{select }u]=\frac{w(u,v)}{\gamma_v}.
	\end{align}
	Similar to the Spontaneous IC Polling, to select $u$, we compute $\Pr[A_i]$ as the probability of node $u_i \in N^{in}(v)$ being selected as the first node,
	\begin{align}
	\label{eq:probn1}
	\Pr[A_i]=\frac{w(u_i,v)\prod_{j = 1}^{i-1}(1-w(u_j,\src(R_j)))}{\gamma_v}.
	\end{align}
	%	\item[3)] The $\src(R_j)$ is excluded from $R_j$.
\end{itemize}
\begin{algorithm} \small
	\caption{\ROS{} Sketch Sampling Scheme}
	\label{alg:eris}
	\KwIn{Graph $\G = (V,E,w)$}
	\KwOut{A random \ROS{} $R_j$}
	Pick a node $v$ by importance sampling with the prob. of selecting node $u$ given by Eq.~\ref{eq:probu};\\
	Select one in-neighbor $u_i$ of $v$, $u_i \in I_N(v)$, with probability of selecting $u_i$ given in Eq.~\ref{eq:probn};\\
	Initialize a queue $Q = \{v_i\}$, $R_j = \{v,u_i\}$;\\
	Select $u_t \in I_N(v), \forall t > i$ to $Q, R_j$ with probability $w(u_j, v)$;\\
	\While{$Q$ not empty}{
		$v = Q.\textsf{pop}()$;\\
		\For{$u \in N^{in}(v)\backslash (R_j \cup Q)$}{
			\If{$\textsf{rand}() \geq w(u,v)$}{
				$R_j \leftarrow R_j \cup \{u\}$;\\
				$Q.\textsf{push}(u)$;\\
			}
		}
	}
	\textbf{return} $R_j$;
\end{algorithm}
The two modifications guarantee that the generated \ROS{} is non-empty making it more efficient in estimating outward influences since the empty ones never intersect with any set of nodes. The detailed description of \ROS{} sampling is shown in Alg.~\ref{alg:eris}.

The first two steps in Alg.~\ref{alg:eris} follows the modifications 1 and 2 in \ROS{} and the rest of the procedure performs similarly as for \RIS{} \cite{Borgs14}. Note that step 4 only adds the selected neighbors $u_i$ of $v$ into $Q$ but adds both $v$ and the $u_i$ to $R_j$. The loop from Line~5-10 mimics the behavior of \RIS{} by probabilistically sampling the reverse influenced nodes.

We establish the following important lemma that connects our \ROS{} samples with the outward influence of a set $S$.
\begin{Lemma}
	\label{lem:comp_ext}
	Given a random \ROS{} sample $R_j$ generated from the stochastic graph $\G = (V,E,w)$, for a set $S \subseteq V$ of nodes, the following equality holds,
	\begin{align}
	\label{eq:compute_pr_ie}
	\I_E(S) = \Pr[R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S] \cdot \Gamma,
	\end{align}
	where $\Gamma = \sum_{v \in V}\gamma_v$.
\end{Lemma}
\begin{proof} 
	Given a stochastic graph $\G$, recall that $\Omega_\G$ is the space of all possible sample graphs $g \sim \G$ and $\Pr[g]$ to be the probability that $g$ is realized from $\G$. In a realization $g \in \Omega_\G$, $\eta_g(S,v)$ has value 1 if $v$ is reachable from $S$ in $g$ and $v \notin S$. Then from the definition of $\I_E(S)$ in Eq.~\ref{eq:compute_ie}, we have,
	\begin{align}
	\I_E(S)& = \sum_{g \in \Omega_\G} \eta_g(S) \Pr[g] = \sum_{g \in \Omega_\G} \sum_{v \in V} \eta_g(S,v) \Pr[g] \nonumber \\
	& = \sum_{g \in \Omega_\G} \Big ( \sum_{v \in V\backslash S} \eta_g(S,v) \Pr[g] + \sum_{v \in S} \eta_g(S,v) \Pr[g] \Big ) \nonumber \\
	& = \sum_{g \in \Omega_\G} \sum_{v \in V\backslash S} \eta_g(S,v) \Pr[g] = \sum_{v \in V\backslash S} \sum_{g \in \Omega_\G} \eta_g(S,v) \Pr[g] \nonumber
	\end{align}
	\normalsize
	Let consider the graph sample space $\Omega_\G$, based on a node $v \in V \backslash S$, we can divide $\Omega_\G$ into two partitions: 1) $\Omega^\emptyset_\G(s)$ contains those samples $g$ in which $v$ has \textit{no incoming edges}; and 2) $\bar \Omega^\emptyset_\G(s) = \Omega \backslash \Omega^\emptyset_\G$. However, for $g \in \Omega^\emptyset_\G$, $\eta_g(S,v) = 0$ for any $v \in V \backslash S$. Thus, we obtain,
	\begin{align}
	\I_E(S) & = \sum_{v \in V\backslash S} \Big ( \sum_{g \in \Omega^\emptyset_\G} \eta_g(S,v) \Pr[g] + \sum_{g \in \bar \Omega^\emptyset_\G} \eta_g(S,v) \Pr[g]\Big ) \nonumber \\
	& = \sum_{v \in V\backslash S} \sum_{g \in \bar \Omega^\emptyset_\G} \eta_g(S,v) \Pr[g].
	\end{align}
	We define $\bar \Omega^\emptyset_\G(s)$ to be a new probability space in which a sampled graph $\bar g \in \Omega^\emptyset_\G(s)$ has probability $\Pr[\bar g] = \frac{\Pr[\bar g \in \Omega_\G]}{\gamma_v}$. In the new space, we have,
	\begin{align}
	\I_E(S) & = \sum_{v \in V\backslash S} \sum_{\bar g \in \bar \Omega^\emptyset_\G} \eta_{\bar g}(S,v) \Pr[\bar g] \gamma_v.
	\end{align}
	Observe that since the graph $\bar g \in \bar \Omega^\emptyset_\G(s)$ has non-empty neighbors of node $v$, we can construct a \ROS{} sample $R_j(\bar g,v)$ with $\src(R_j(\bar g,v)) = v$ containing all the nodes reachable to $v$ in $\bar g$. Moreover, $\eta_{\bar g}(S,v)$ represents the event that $R_j(\bar g,v)$ intersects with $S$, $R_j(\bar g,v) \cap S \neq \emptyset$. Thus,
	\begin{align}
	\I_E(S) & = \sum_{v \in V\backslash S} \sum_{\bar g \in \bar \Omega^\emptyset_\G} \textbf{1}_{R_j(\bar g, v) \cap S \neq \emptyset} \Pr[\bar g] \gamma_v \nonumber \\
	& = \sum_{v \in V\backslash S} \Pr[R_j(v) \cap S \neq \emptyset] \gamma_v \nonumber \\
	%		& = \sum_{v \in V\backslash S} \Pr[R_j(v) \cap S \neq \emptyset] \frac{\gamma_v}{\gamma_0} \cdot \gamma_0 \nonumber \\
	& = \sum_{v \in V\backslash S} \Pr[R_j(v) \cap S \neq \emptyset] \frac{\gamma_v}{\sum_{u \in V} \gamma_u} \cdot \sum_{u \in V} \gamma_u \nonumber \\
	& = \sum_{v \in V\backslash S} \Pr[R_j(v) \cap S \neq \emptyset] \Pr[\src(R_j) = v] \cdot \Gamma \nonumber \\
	& = \Pr[R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S] \cdot \Gamma.
	\end{align}
	That completes the proof.
\end{proof}
In other words, Lemma~\ref{lem:comp_ext} states that instead of computing or estimating the outward influence $\I_E(S)$ directly, we can equivalently compute or estimate $\Pr[R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S]$. We can get back $\I_E(S)$ by multiplying $\Pr[R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S]$ by a constant $\gamma_0 \cdot n$.

\subsubsection{Sketch-based Outward Influence Oracle}

As shown in Lemma~\ref{lem:comp_ext}, the outward influence $\I_E(S)$ can be estimated through $\Pr[R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S]$. For a random \ROS{} sample $R_j$ and a set of nodes $S$, we define an associated random variable $X_j(S)$ as follows,
\newcommand{\twopartdef}[3]
{
	\left\{
	\begin{array}{ll}
		#1 & \mbox{if } #2 \\
		#3 & \mbox{otherwise}
	\end{array}
	\right.
}
\begin{align}
\label{eq:varx}
X_j(S) = \twopartdef {1} {R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S} {0}
\end{align}
Thus, we have,
\begin{align}
\E[X_j] = \Pr[R_j \cap S \neq \emptyset \wedge \src(R_j) \notin S] = \frac{\I_E(S)}{\gamma_0 \cdot n}.
\end{align}

%Furthermore, the probability $\Pr[R_j \cap S \neq \emptyset]$ can be estimated by sampling multiple \ROS{} samples and taking average over random variables $X_j(S)$ defined as follows,
%
%and when the context is clear, we also use $X_j$ for $X_j(S)$.
%
%Our \SkEIE{} algorithm utilizes the optimal Stopping rule-based Monte-Carlo estimation in \cite{Dagum00} combined with \ROS{} sampling to provide an $(\epsilon,\delta)$-approximation of $\I_E(S)$ where $\epsilon, \delta$ can be arbitrarily small. That is \SkEIE{} returns an approximate value $\hat \I_E(S)$ of $\I_E(S)$ satisfying,
%\begin{align}
%	\label{eq:eps-del}
%	\Pr[|\hat \I_E(S) - \I_E(S)| \leq \epsilon \I_E(S)] \geq 1-\delta
%\end{align}
%
%The detailed description of \SkEIE{} algorithm is presented in Alg.~\ref{alg:skeie}.
%
%%\todo{Replace with the algorithm to generate the reverse sample}
%
%\begin{algorithm} \small
%	\caption{\SkEIE{} algorithm}
%	\label{alg:skeie}
%	\KwIn{Graph $\G = (V,E,w)$, a set $S$ and $\epsilon,\delta$}
%	\KwOut{An $(\epsilon,\delta)$-approximate of $\I_E(S)$}
%	Compute $\Upsilon = 1+(2+2\cdot \epsilon/3)\ln (2/\delta)/\epsilon^2$;\\
%	Initialize $h = 0, T = 0$;\\
%	\While{$h \leq \Upsilon$}{
%		Generate a random \ROS{} $R_j$\tcp*{Algorithm~\ref{alg:eris}}
%		$T \leftarrow T+1$;\\
%		\If{$R_j \cap S \neq \emptyset$}{
%			$h \leftarrow h + 1$;\\
%		}
%	}
%	\textbf{return} $\hat \I_E(S) = h/T \cdot \sum_{v \in V}\big(1-\prod_{u \in N^{in}(v)}(1-w(u,v))\big)$;
%\end{algorithm}
%
%The Algorithm~\ref{alg:skeie} first computes the threshold $\Upsilon$ at which if we see that number of random \ROS{} intersecting with $S$, we are certain that the resulting estimation is good enough. The main component in our algorithm is a loop which iteratively generates a \ROS{} $R_j$ and check whether it intersects with the set $S$. If so, the number of intersecting \ROS{} increases by 1 up to the threshold $\Upsilon$. Finally, after satisfying the stopping condition on intersecting \ROS{}, the algorithm returns an $(\epsilon,\delta)$-approximate of $\I_E(S)$.
%
%The approximation guarantee of \SkEIE{} is followed from Stopping Rule Theorem in \cite{Dagum00} and stated in the following theorem.
At this point, we can apply the Monte-Carlo estimation algorithm \cite{Dagum00} to obtain an $(\epsilon,\delta)$-approximate of $\I_E(S)$. In particular, we utilize \ROS{} sampling to generate a large enough collection $\R$ of $T$ \ROS{} samples, $\R = \{R_1, \dots, R_T\}$ and obtain an estimate $\hat \I_E(S)$ for any set $S$ by,
\begin{align}
\hat \I_E(S) = \frac{\Cov_\R(S)}{T} \cdot \gamma_0 \cdot n,
\end{align}
where $\Cov_\R(S)$ is the number of \ROS{} samples in $\R$ not rooting from nodes in $S$ and intersecting with $S$, i.e.,
\begin{align}
\Cov_\R(S) = |\{R_j \in \R | R_j \cap S \neq \emptyset \wedge \src(R_j \notin S)\}|
\end{align}

Thus, applying the Monte-Carlo algorithm in \cite{Dagum00} gives,
\begin{theorem}
	Given a set $S\subseteq V$, a stochastic graph $\G = (V,E,w)$ and precision parameters $\epsilon,\delta$, the Monte-Carlo algorithm on \ROS{} samples guarantees that,
	\begin{align}
	\Pr[(1-\epsilon)\I_E(S) \leq \hat \I_E(S) \leq (1+\epsilon)\I_E(S)] \geq 1-\delta,
	\end{align}
	and the number of generated \ROS{} satisfies,
	\begin{align}
	\E[T] \leq O(\ln (\frac{2}{\delta}) \frac{1}{\epsilon^2} \frac{1}{\E[X_j]}).
	\end{align}
\end{theorem}
Thus, to build an oracle for outward influence estimation, we will generate multiple \ROS{} samples in the preprocessing step and return $\hat \I_E(S)$ for any queried set $S$.
